Correspondence-Free, Function-Based Sim-to-Real Learning for Deformable Surface Control

This paper presents a correspondence-free, function-based sim-to-real learning method for controlling deformable freeform surfaces. Unlike traditional sim-to-real transfer methods that strongly rely on marker points with full correspondences, our approach simultaneously learns a deformation function space and a confidence map -- both parameterized by a neural network -- to map simulated shapes to their real-world counterparts. As a result, the sim-to-real learning can be conducted by input from either a 3D scanner as point clouds (without correspondences) or a motion capture system as marker points (tolerating missed markers). The resultant sim-to-real transfer can be seamlessly integrated into a neural network-based computational pipeline for inverse kinematics and shape control. We demonstrate the versatility and adaptability of our method on both vision devices and across four pneumatically actuated soft robots: a deformable membrane, a robotic mannequin, and two soft manipulators.

==> tex/TabDifferentKernels.tex <==
\begin{table}[t] \scriptsize %\tiny %scriptsize
%\footnotesize
\centering
\caption{Impact of the Number of Kernels\Tian{Not Table, Bar Chart}}\label{tab:DiffKernels}
% \jun{Should modify to coherent with three categories definition}
\begin{tabular}{c|c|c|c|c}         %adjust column number 
\hline \hline                       %horizontal line
% \specialrule{0em}{2pt}{1pt}         %vertical space


\multicolumn{1}{c|}{\multirow{2}{*}{Case No.}} & \multicolumn{1}{c|}{\multirow{2}{*}{\# of Kernel}} & \multicolumn{1}{c|}{Ave. Err.}& \multicolumn{1}{c|}{Max. Err.}& \multicolumn{1}{c}{Computational Cost (ms)}\\ %column arrangement

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{(mm)}& \multicolumn{1}{c|}{(mm)}& \multicolumn{1}{c}{with $10^5$ Space Warping}\\ %column arrangement

% \specialrule{0em}{1pt}{2pt}
\hline \hline
% \specialrule{0em}{2pt}{2pt}


%Case I
\multicolumn{1}{c|}{

\multirow{4}{*}{Case I}

}  & \multicolumn{1}{c|}{10}  
& \multicolumn{1}{c|}{3.18}  & 
\multicolumn{1}{c|}{13.08}  & 
\multicolumn{1}{c}{16.67}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{34}  & \multicolumn{1}{c|}{2.23}  & 
\multicolumn{1}{c|}{13.37} & 
\multicolumn{1}{c}{58.35}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{100}  & \multicolumn{1}{c|}{1.72}  & 
\multicolumn{1}{c|}{12.92}& 
\multicolumn{1}{c}{144.54}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{200}  & \multicolumn{1}{c|}{1.70}  & 
\multicolumn{1}{c|}{13.33} & 
\multicolumn{1}{c}{294.45}  \\

\cline{1-5}  





%Case II
\multicolumn{1}{c|}{

\multirow{4}{*}{Case II}

}  & \multicolumn{1}{c|}{10}  & \multicolumn{1}{c|}{1.53}  & 
\multicolumn{1}{c|}{10.75}  & 
\multicolumn{1}{c}{17.58} \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{34}  & \multicolumn{1}{c|}{1.26}  & 
\multicolumn{1}{c|}{11.28} & 
\multicolumn{1}{c}{60.81}   \\
\cline{2-5} 

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{100}  & \multicolumn{1}{c|}{0.97}  & 
\multicolumn{1}{c|}{10.50} & 
\multicolumn{1}{c}{151.17}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{200}  & \multicolumn{1}{c|}{0.92}  & 
\multicolumn{1}{c|}{10.73}  & 
\multicolumn{1}{c}{285.51} \\

\cline{1-5}  

%Case III
\multicolumn{1}{c|}{

\multirow{4}{*}{Case III}

}  & \multicolumn{1}{c|}{10}  & \multicolumn{1}{c|}{1.74}  & 
\multicolumn{1}{c|}{9.62} & 
\multicolumn{1}{c}{15.39}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{34}  & \multicolumn{1}{c|}{1.36}  & 
\multicolumn{1}{c|}{9.92}  & 
\multicolumn{1}{c}{59.81} \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{100}  & \multicolumn{1}{c|}{1.23}  & 
\multicolumn{1}{c|}{9.55}& 
\multicolumn{1}{c}{148.67}  \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{200}  & \multicolumn{1}{c|}{1.20}  & 
\multicolumn{1}{c|}{9.71} & 
\multicolumn{1}{c}{291.18}  \\

\cline{1-5}  

%Case IV
\multicolumn{1}{c|}{

\multirow{4}{*}{Case IV}

}  & \multicolumn{1}{c|}{10}  & \multicolumn{1}{c|}{1.98}  & 
\multicolumn{1}{c|}{10.83}  & 
\multicolumn{1}{c}{14.98}  \\
\cline{2-5} 

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{34}  & \multicolumn{1}{c|}{1.65}  & 
\multicolumn{1}{c|}{11.74} & 
\multicolumn{1}{c}{57.48}   \\
\cline{2-5}   

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{100}  & \multicolumn{1}{c|}{1.29}  & 
\multicolumn{1}{c|}{11.11} & 
\multicolumn{1}{c}{152.61} \\
\cline{2-5}  

\multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{200}  & \multicolumn{1}{c|}{1.32}  & 
\multicolumn{1}{c|}{10.94}& 
\multicolumn{1}{c}{298.91}  \\

\cline{1-5}  


% \specialrule{0em}{0pt}{2pt} 
\hline\hline
\end{tabular}
\footnotesize 
\label{tab:DiffMorphingSystems}
\vspace{5pt}
\end{table}


==> tex/secIntroduction.tex <==
\section{Introduction}\label{secIntro}
Soft robotic systems have demonstrated the ability to dynamically adapt their shapes in response to programmed actuation or environmental stimuli. Existing prototypes were developed for haptic interfaces (ref.~\cite{inForm2013UIST,Stanley2015CtrlSurf,Bryan2019SoRoInterface,koehler2020model,Je2021ElevateAW})\JENew{~and soft manipulators (ref.~\cite{della2020model,Thomas2019TRO, Renda2014TRO}). Many of these soft robotic systems have realized deformable free-form surfaces -- e.g., a soft robotic mannequin} developed in~\cite{Tian2022SoRoMannequin}, which is driven by pneumatic actuators to mimic the front shapes of different human bodies. 
%Moreover, for the fabrication of customized garments, a soft robotic mannequin with deformable free-form surface has been developed in~\cite{Tian2022SoRoMannequin}, which is driven by pneumatic actuators to mimic the front shapes of different human bodies on the same mannequin.
%
\JENew{
However, the shape control of deformable freeform surfaces is still an unsolved challenging issue in soft robotics, which is mainly caused by the infinite \textit{degrees-of-freeform} (DoFs) deformation embedded in the elastic body of a soft robot. Details will be discussed below.
%%Numerical simulation is usually employed to establish the mapping $\mathcal{S}(\mathbf{a})$ between the actuation parameters $\mathbf{a}$ and the deformed shapes $\mathcal{S}$ \cite{fangICRA,Goury2018TRO}. The differentiation of this forward kinematic mapping is usually employed to solve the \textit{inverse kinematic} (IK) problem for determining the actuation parameters that can realize a target shape $\mathcal{S}^t$. This is usually formulated as an optimization problem to iteratively run a simulator to determine the optimal actuation $\mathbf{a}_{opt}$ that minimizes the difference between $\mathcal{S}(\mathbf{a}_{opt})$ and $\mathcal{S}^t$ (ref.~\cite{Guoxin2020TRO}). 
}

%simulation plays a crucial role in establishing the mapping between the actuation parameters and the deformed shapes. The differentiation of this forward kinematic mapping is usually employed to solve the inverse kinematic problem for determining the actuation parameters that can realize a target shape. However, the free-form surfaces obtained from the simulators are always different from the physically deformed shapes due to the errors introduced by the hardware and the simplification adopted in the physical simulation. To fill the gap, we propose a novel sim-to-real learning method based on deformation functions that can map the geometric shape of a simulated model into the corresponding shape of the physical model. Unlike existing sim-to-real learning methods that rely on completely acquired dense markers, our method accommodates sparsely distributed markers and can resiliently use all captured frames, even for those in the presence of missing markers. Additionally, our sim-to-real method can process dense point clouds from imperfect scans, even in the absence of point correspondence. The effectiveness and versatility of this approach have been demonstrated on three different types of surface-based robots, including the deformable membrane, soft manipulator, and soft robotic mannequin. Furthermore, our sim-to-real method has been integrated into a neural network-based computational pipeline designed to tackle the inverse kinematic problem\TianModify{ on a pneumatically actuated deformable mannequin}{ on general surface-based deformable robots}.

\subsection{Kinematics for Shape Control}\label{subsecIntroShapeCtrl}
An essential shape control problem of soft robotics is to compute the actuation (denoted by a vector $\mathbf{a}$) that can drive the free-form surface $\mathcal{S}$ to approach a target shape $\mathcal{S}^t$. It presents much higher DoFs compared to the \textit{inverse kinematics} (IK) problems for articulated robots. The high DoFs lead to high complexity in both the forward shape estimation (i.e., predicting the resultant shape $\mathcal{S}$) and the IK computation to determine the values of $\mathbf{a}$. Earlier works have been developed to conduct an iteration-based IK solver with Jacobian physically evaluated on hardware setup~\cite{Tian2022SoRoMannequin, Yip2014TROHardwardGradient}. However, this approach suffers from high costs in both computation and data acquisition. Additionally, its performance is unstable as the Jacobian evaluation is highly dependent on the accuracy of shapes captured on the physical setup, which is hard to be guaranteed in practice. 

In the existing research works of kinematics computing for deformable objects, high DoFs in the configuration space are typically modeled either by reduced analytical models or by discrete numerical models. Comprehensive reviews can be found in \cite{Renda2023TROModeling,arriola2020modeling}. Reduced analytical models are often used for soft manipulators with bending deformation (e.g., ref. \cite{marchese2016design,Thomas2019TRO}), where the surface deformation is trivial in general. \JENew{Differently, numerical simulation is usually employed to establish the mapping $\mathcal{S}(\mathbf{a})$ between the actuation parameters $\mathbf{a}$ and the deformed freeform shapes $\mathcal{S}$ (ref.~\cite{fangICRA,Goury2018TRO,du2021_diffpd,hu2019chainqueen}). The differentiation of this forward kinematic mapping is usually employed to solve the IK problem for determining the actuation parameters $\mathbf{a}$ that can realize a target shape $\mathcal{S}^t$. This is usually formulated as an optimization problem to iteratively run a simulator to determine the optimal actuation $\mathbf{a}_{opt}$ that minimizes the difference between $\mathcal{S}(\mathbf{a}_{opt})$ and $\mathcal{S}^t$ (ref.~\cite{Guoxin2020TRO}).}

However, numerical simulation in general cannot be computed efficiently enough to realize a fast IK solver. A widely adopted strategy to mitigate the issue of efficiency is to first collect a dataset using the numerical solution and train a \textit{neural network} (NN) for the forward shape estimation of the deformable object (e.g., ref.~\cite{Thomas2018SoRoCtrlReview, bern2020soft, Fang2022Sim2Real}). 

\subsection{Challenges of Sim-to-Real Transfer}\label{subsecIntroSim2Real}
\JENew{
Subsequently, the free-form surfaces predicted by a simulator can differ from the physically deformed shapes due to errors introduced by hardware and simplification in numerical simulations. This difference can be significant during large deformation of a soft robot's freeform surface (see Fig.\ref{fig:motivation} for an example). A sim-to-real network can be trained to bridge this gap using marker points obtained from physical experiments by a motion capture system -- e.g., the earlier works presented in \cite{Zhang2022Sim2RealSoRoFish,Dubied2022Sim2RealFEM,Fang2022Sim2Real}. However, this sim-to-real method relies on marker data with full correspondence, limiting its ability to compensate for only a limited number of positions rather than larger surface areas. For instance, only the position of the end effector is corrected in \cite{Fang2022Sim2Real}, not the shape of the entire soft manipulator. When missing data occurs -- often due to vision occlusion caused by significant deformation -- the frames with missing markers cannot be used as the input for sim-to-real learning (see Fig.\ref{fig:motivation}(a) for an example). As a consequence, shape errors during large deformations cannot be accurately captured. Furthermore, this sim-to-real method also restricts the use of other devices, such as 3D scanners, for sim-to-real learning since there is generally no point correspondence provided in the scanned point clouds (see Fig.\ref{fig:motivation}(b) for an example).} 


%The research work presented in this paper is to realize a similar function of soft deformable robot\rev{}{, which is to serve as a reusable mould with programmable shape for sustainable garment fabrication (e.g.,~\cite{morby2016,parkes_2022})}.
%Specifically, by giving a target shape of an individual as $\mathcal{S}^t$, the deformable mannequin is expected to deform into a shape $\mathcal{S}$ that minimizes the shape difference (see Fig.\ref{fig:motivation}(a) for examples). The geometric errors are evaluated by capturing the deformed shapes of the robotic mannequin with the help of a structure-light based 3D scanner (see Fig.\ref{fig:motivation}(b)). Shape control of a deformable free-form surface is challenging, and the reasons for this are analyzed below with a review of related work in the literature.
%\rev{}{The proposed deformable mannequin system has the potential to assist garment design that requires a perfect fit in full body shape, such as bespoke items and wetsuits. Additionally, we will explore its application in serving as a reusable deformable mold for sustainable garment fabrication~\cite{morby2016,parkes_2022}.}
% Moreover, numerical simulation invariably exhibits a prediction error compared to physical performance, a discrepancy often referred to as the `reality gap'~\cite{rss2020Sim2Real}.
%
%Subsequently, NN-based sim-to-real transfer~\cite{Dubied2022Sim2RealFEM, Zhang2022Sim2RealSoRoFish, Iyengar2023Sim2RealCTR, Fang2022Sim2Real} is applied to achieve high precision while maintaining reasonable efficiency in data acquisition -- i.e., only a small set of physical data is needed. When both the forward kinematic computing and the sim-to-real transfer are realized by neural networks, the gradients of IK objectives can be efficiently and effectively computed by differentiating the networks~\cite{}. In short, fast IK can be achieved. 

\begin{figure}[!t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figTeaser.jpg}\\
\vspace{-5pt}
\caption{Motivation and challenges. 
\JENew{(a) On a soft robotic mannequin with nine air chambers, the simulated shape exhibits distributed approximation errors, visualized by a color map. When using a motion capture system to collect marker positions for sim-to-real correction, two markers were missed on the belly due to vision occlusion caused by significant deformation in the belly region. 
(b) Large geometric discrepancies between simulation and reality are also observed on a soft manipulator composed of 6 chambers. When a 3D scanner is used to capture dense point clouds of the manipulator’s real shape, the conventional sim-to-real approach cannot be applied due to the lack of known correspondence between the scanned point clouds. }
}\label{fig:motivationBackup}
\end{figure}

%While the sim-to-real approach has been developed for controlling robots with compliance~\cite{Iyengar2023Sim2RealCTR,shah2021soft} and for deformable object manipulation~\cite{Fei2021ICRASim2Real,liang2023real} with the ground-truth information maintaining fixed~\cite{Mehrnoosh2022MarkerSim2Real,peng2018sim}  or dense~\cite{Rika2022BaySim2Real,Fei2021ICRASim2Real,liang2023real} degrees of freedom, less effort has been focused on the sim-to-real problem on free-form surfaces using sparse and incomplete sets of markers. \Tian{Is this appropriate?}
%
%\Guoxin{Sim-to-real approaches have been developed for controlling robots with compliance~\cite{Iyengar2023Sim2RealCTR,shah2021soft} and for deformable object manipulation~\cite{Fei2021ICRASim2Real,liang2023real}. These works generally adopt rich physical information obtained from well-captured frames with constant DOFs as training data. Less effort has been focused on the sim-to-real problem on free-form surfaces using sparse and incomplete sets of markers. However, ...}

%\charlie{Suggest to change as follows:}
%
%Sim-to-real approaches have been developed for controlling robots with compliance~\cite{Iyengar2023Sim2RealCTR,shah2021soft} and for deformable object manipulation~\cite{Fei2021ICRASim2Real,liang2023real}. These works generally adopt rich physical information obtained from well-captured frames with constant DOFs as training data. Less effort has been focused on the sim-to-real problem on free-form surfaces using sparse and incomplete sets of markers. 
%
%There is an effort to use a 3D scanner to directly obtain the surface shapes as point clouds~\cite{Forte2022InverseDesignMembrane}, which however suffers from the problems of inefficiency and unstable boundary regions. Moreover, the scanned shapes at different time currents have no correspondence with each other, which needs a lot of extra effort for non-rigid registration~\cite{deng2022survey}.
%
%Using a motion capture system can precisely capture the position of markers attached to a free-form surface~\cite{Mehrnoosh2022MarkerSim2Real, scharff2021sensing}. %Mehrnoosh2022MarkerSim2Real
%However, only sparse data can be obtained, representing a reduced order of information on the shape of the free-form surface. The motion capture system can also suffer from the problems of marker missing due to camera view occlusion -- especially when large deformation is presented (see Fig.\ref{fig:motivation}(b, c) for an example). 


% a corrected model $\mathcal{S}^*$

\begin{table*}[t]
\footnotesize
\centering
\caption{\rev{}{List of Notations}}\label{tab:Symbols}
\begin{tabular}{cl|cl}
\hline \hline
\specialrule{0em}{2pt}{1pt}
Symbol & Description  & Symbol & Description  \\ 
\specialrule{0em}{1pt}{1pt} \hline \specialrule{0em}{1pt}{2pt}

% first line 
$ \mathbf{a} $  & Actuation parameters (i.e., chamber pressures)
&  $\mathcal{S}^t$  & The target body shape to be achieved by IK \\

% second line
$\mathcal{S}$ & The simulated shape of the deformable surface & 
 $\mathcal{S}^*$  & The corrected shape obtained from our \textit{sim-to-real} method \\

% third line
$\mathcal{S}^c$ & The compact shape descriptor (i.e., control points) of $\mathcal{S}$ &
 $\mathcal{S}^p$    & The scanned 3D shape on the physical setup \\

% forth line
 $\mathcal{N}_{fk}$ & Forward kinematics network that predicts $\mathcal{S}^c$ from $ \mathbf{a} $ & $\mathcal{N}_{mk}$& The baseline network predicting positions of markers \\

% fifth line
 $\mathcal{N}_{rbf}$ & Function prediction network that predicts $\bm{\gamma}$ by $\mathcal{S}^c$ &  $\mathcal{N}_{s2r}$& Combination of $\mathcal{N}_{rbf}$ and $\bm{\Phi}(\cdot)$  \\

% sixth line
$\bm{\Phi}(\cdot)$ & The space warping function used to deform $\mathcal{S}$ to $\mathcal{S}^*$ & 
$\bm{\gamma} = [\bm{\alpha}_{0}, \ldots \bm{\beta}_i]$ & Variables to determine the function space
\\ 

%$\bm{\gamma} = [\bm{\alpha}_0, \bm{\alpha}_1, ...  \bm{\beta}_i]$ are variables of function space
% seventh line
$\{ \mathbf{q}_i \}$& Centers of Gaussian kernels (also markers on $\mathcal{S}$) in $\bm{\Phi}(\mathbf{p})$ & $\mathbf{p}$, $\mathbf{p}^* \in \mathbb{R}^{3}$ & The surface point on $\mathcal{S}$ and $\mathcal{S}^*$ respectively \\

%eighth line
% $\mathbf{c}^*$ is the closet point of $\mathbf{p}^*$ on the target shape $\mathcal{S}^t$
$(\mathbf{R},\mathbf{t})$ & Rotation matrix and translation vector to re-pose $\mathcal{S}^t$&
$\mathbf{c}^*$  & Closet point of $\mathbf{p}^*$ on $\mathcal{S}^t$ \\

% $\mathcal{S}^c=\mathcal{N}_{fk}(\mathbf{a})$.

% eighth line
%$\mathcal{N}_{s2r}$& Consisting of $\mathcal{N}_{rbf}$ and $\bm{\Phi}(\cdot)$ & $\mathcal{N}_{mk}$& The baseline network predicting complete sets of markers\\
$(u_p,v_p)$ & A point in the parametric domain of B-spline surface &
$\mathbf{B}(\cdot)$ & B-Spline function as decoder mapping $(u_p,v_p)$ to $\mathbf{p}$\\


\specialrule{0em}{1pt}{1pt} \hline\hline
\end{tabular}\label{table_variable}
\end{table*}


\subsection{Our Method}
\JENew{We propose a function-based learning method to tackle the sim-to-real challenges outlined above. Our method is designed to handle diverse types of input data, including 1) motion capture frames with missing markers and 2) scanned dense 3D point clouds without correspondence. The trained sim-to-real module can be seamlessly integrated into a neural network-based fast IK computing pipeline for shape control.}
%To facilitate the neural network-based fast IK computing, we propose a resilient sim-to-real learning method, which can fully leverage the entire dataset of sparse marker positions obtained from the physical setup. 
It is a new learning architecture that learns the function space of shape deformation represented by \textit{radial basis functions} (RBF). Specifically, each simulated free-form surface is approximated by a B-spline surface, the control points of which are employed as the shape descriptor in a lower dimension. The input of our sim-to-real network is the control points of a simulated body shape, and the output is the coefficients of RBFs that define a spatial warping function $\bm{\Phi}(\mathbf{p})$ by using the positions of `virtual' markers as kernel centers. The sim-to-real network can be trained from sparse and even incompletely captured sets of markers. \JENew{When dense 3D point clouds are employed for sim-to-real learning, non-rigid registration is conducted to find the corresponding `markers' on the point clouds according to the prescribed markers on the simulated models. By these `virtual' correspondences -- although not as accurate as the positions of physical markers, our sim-to-real network can still be trained to give shape approximation with high quality.}

The space warping function $\bm{\Phi}(\mathbf{p})$ is in a closed-form and gives a continuous mapping from the shape of a simulated model to the shape of a corrected model that matches the reality. Working together with the forward kinematics prediction that is trained by simulation, this forms an end-to-end NN-based pipeline that can accurately predict the physical shapes of robotic deformable surfaces. This computation pipeline is analytically differentiable so that the gradient-based iteration for IK can be computed efficiently \JENew{(details are given in Appendix \ref{AppendixIKAlg} and \ref{AppendixDifferentiation}).} The quality of IK solutions has been verified by scanning the physical shape $\mathcal{S}^p$ to compare with the input target shape $\mathcal{S}^t$. All notations used in this paper are summarized in Table \ref{tab:Symbols}. 

The technique contributions of our work are summarized as follows:
%Here, we present a free-form surface system with improved design compared to~\cite{Tian2022SoRoMannequin}, ensuring shape morphing function to a wide range of human body shapes on both the front and back sides. The deformable free-form surface is pneumatically driven, and its design and function can be seen in Fig.~\ref{fig:Teaser}(a).
%
%\begin{itemize}
%\item A resilient sim-to-real learning method for deformable free-form surfaces that can employ sparse and incomplete sets of markers to bridge the reality gap by RBF-based spatial warping functions;
%
%\item A neural network-based method that can efficiently solve the inverse kinematics problem with its performance physically verified on a pneumatically actuated deformable mannequin. 
%\end{itemize}
%
\begin{itemize}
\item %\TianModify{}{A general sim-to-real learning method for deformable free-form surfaces that can employ either sparse and incomplete sets of markers, or dense point clouds, even in the absence of point-to-point correspondence, to bridge the reality gap by RBF-based spatial warping functions;}
\JENew{A resilient sim-to-real learning method for deformable free-form surfaces that bridges the reality gap through RBF-based spatial warping functions, effectively utilizing either sparse \& incomplete marker sets or dense point clouds without correspondence;}

\item %\TianModify{}{A neural network-based method that can efficiently solve the inverse kinematics problem with its performance physically verified on a pneumatically actuated deformable mannequin. }
\JENew{A compatibility constraint as a regularization loss that improves the method’s capability to handle models with large deformations;}
%meshes of varying densities and to support simulators with differing accuracy levels;}

\item %\TianModify{}{The compatible constraint is further proposed as a penalty term to enhance the function space learning, facilitating the capability to handle meshes (that describe the morphology of robots) of varying densities and simulators with different accuracy levels. The effectiveness and versatility of our pipeline have been verified on three different surface-based deformable robots.}
\JENew{A neural network-based method that can efficiently solve the inverse kinematics problem for shape control in soft deformable robots.}
\end{itemize}
%Experimental tests were conducted on a variety of individual shapes presented in the CAESAR dataset~\cite{CAESAR2002}. The shape approximation errors were physically evaluated on a deformable mannequin with 1:2 ratio to the full size. 
\JENew{The effectiveness of our sim-to-real learning and the resultant fast IK solver has been verified on three pneumatically actuated soft robots, including a
deformable membrane, a soft manipulator, and a deformable robotic mannequin.} 
%The average shape approximation errors on all tested individuals are less than $3.1$ mm on a deformable mannequin with 1:2 ratio to the full size. 
%The detailed statistics are given in the supplementary document. 

\JENew{This article is an extension of our preliminary work presented in~\cite{Tian-RSS-24} with significant improvement to support more general robotic hardware and general input device as 3D scanners. In particular, we have made the following improvements: 1) a new loss as a regularization term for compatibility constraint, 2) a new method to incorporate the dense point clouds as input for sim-to-real learning, 3) verification and experimental tests on two more general soft robots -- including a deformable membrane and a soft manipulator.}

==> tex/secResult.tex <==
\section{Implementation Details and Results}\label{secResult}
We have implemented the proposed approach in C++ and Python. The network training phase is implemented on the PyTouch platform with the batch size as $32$, the learning rate at $0.001$ and the maximum number of epochs as $150$. 
%Backpropagation is all realized by analytical differentiation of networks. \charie{why hide?}
For the \TianModify{interference}{inference} phase, we transferred the trained networks to integrate with our IK solver in C++ running on CPU. The analytical gradients of the networks are employed in our IK solver. \JENew{Our source code will be released on GitHub upon the acceptance of our research submission.} All the training and computational tests are conducted on a PC with Intel i7-12700H CPU, RTX $3060$ GPU and $32$ GB RAM. %\JENew{The results of sim-to-real and fast IK have been verified on the physical setups of three different soft robots.} 

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figHardwareSystem.jpg}
\caption{
%\Tian{make (b) transparent later, should we make (b) larger and make (c) smaller} 
\JENew{Three pneumatic actuated soft robots with large surface deformation are conducted to validate the effectiveness of our sim-to-real approach, including (a) a deformable membrane with 9 chambers, (b) a soft manipulator with two segments -- 3 chambers per segment, (c) a soft robotic mannequin having 15 chambers with 9 independent DoFs,} \TianModify{}{and (d) FlexPAL, which comprises three segments with a total of nine bellows, can undergo substantial compression, inflation, and rotational deformations.}\JENew{Both a motion capture system and a 3D scanner highlighted by red dash line were used in our tests.}
\Tian{Update this figure to add one more setup}
}\label{fig:HardwareSystem}
\end{figure}


\subsection{Hardware for Verification}\label{subsecResHardware}
\JENew{To evaluate the generality of our function-based Sim-to-Real pipeline, we have tested it on three different soft robots (see Fig.\ref{fig:HardwareSystem}), including a deformable membrane, a soft manipulator, and a soft robotic mannequin. An open source pneumatic platform, OpenPneu~\cite{tian2023openpneu}, is used to perform pneumatic actuation on these robots with well-controlled pressures. In addition, two types of vision systems, a Vicon motion capture system~\cite{Vicon} with 8 cameras and an Artec Eva 3D Scanner~\cite{Scanner}, were used for data acquisition for sim-to-real learning. Note that the scanner is also used for capturing ground-truth shapes for validation and the shape errors between the scanned surface and the target shape are measured after applying an ICP-based rigid registration to the target shape. 
}

\subsubsection{Deformable Membrane}\label{secDefMembrane}
\JENew{The first soft robot as shown in Fig.\ref{fig:HardwareSystem}(a) consists of nine chambers that can be inflated independently by pneumatic actuation. Each chamber is covered by a silicone membrane with thickness as 2mm. The dimension of the membrane is 32.0 cm (L) x 32.0 cm (W). By adjusting combinations of air pressure across the nine chambers, the deformable membrane can be shaped into a variety of free-form surfaces~\cite{scharff2021sensing}.}

\subsubsection{Soft Manipulator}\label{secSoftManipulator}
\JENew{The second soft robot for this research is a two-segment soft manipulator \cite{marchese2016design}, with each segment containing three chambers. The total length of the manipulator is 26.0 cm. Rotational deformation in its global structure produces significant shape changes across the robot’s surface, as illustrated in Fig.\ref{fig:HardwareSystem}(b). In existing methods (e.g.,~\cite{webster2010design}), the deformed states of this robot are simplified by only modeling the global structure shape, disregarding the substantial deformation of its outer curved surface. This inaccuracy will lead to problems of realizing the planned collision-free motion on a physical setup. The problem will be effectively solved by using our sim-to-real method.}



\subsubsection{Deformable Mannequin}
\label{secSoftMannequin}
The third robot, shown in Fig. \ref{fig:HardwareSystem}(c), contains a soft robotic mannequin representing both the front and back sides of a human body at a 1:2 scale. \JENew{The total height of the mannequin is 31.5 cm.} It can be deformed by pressurized air and features a design with three layers: an inner soft chamber layer attached to the base solid core, a middle soft chamber layer attached on top of the inner layer, and a top membrane layer (passively morphed) covering the base layers to form the overall smooth shape. \JENew{Detailed design can be found in \cite{Tian2022SoRoMannequin,Tian-RSS-24}.}  
%an inner soft chamber layer attached to the base solid core (for chambers I-III \& V-IX as shown in Fig.\ref{fig:motivation}(a)); a middle soft chamber layer attached on top of the inner layer (as chamber IV in Fig.\ref{fig:motivation}(a)); and a top membrane layer (passively morphed) covering the base layers to form the overall smooth shape. 
By pumping air at varying pressures into the chambers, the soft mannequin can be deformed into different shapes.

%\subsubsection{Actuation and Vision Systems}
%For the actuation system, an open-source pneumatic platform, OpenPneu~\cite{tian2023openpneu}, is employed to control the actuation with well-controlled pressures. There are two vision systems in our experiments including a marker-capturing system and a dense-point-cloud-capturing system. Firstly, a Vicon motion capture system~\cite{Vicon} with 8 cameras is employed to collect the positions of markers on the deformed surfaces, and then a structured-light based 3D scanner Artec Eva Lite~\cite{Scanner} is also utilized to capture the surface geometry of a deformed mannequin as point clouds. The collected information is used to train the Sim-to-Real network. 

\input{tex/TabLearningData}
\begin{figure}[t] 
\centering
\includegraphics[width=0.95\linewidth]{fig/figNNStructureStudy.jpg}\\
\caption{\rev{}{Study of network parameters \JENew{taken on the soft deformable mannequin} -- (a) the maximal shape prediction error w.r.t. different numbers of layers ($h$) and numbers of neurons per layer ($l$) are evaluated to choose the `best' values of $h$ and $l$ for $\mathcal{N}_{fk}$ (circled by black dash lines), and (b) the average shape prediction error w.r.t. the number of neurons in $\mathcal{N}_{rbf}$ is studied to avoid overfitting while training $\mathcal{N}_{s2r}$ using a limited number of samples. Note that $\mathcal{N}_{s2r}$ contains $\mathcal{N}_{rbf}$ plus a space warping module as illustrated in Fig.\ref{fig:sim2RealPipelineOverview}.}}\label{fig:NfkTraining}
\end{figure}

\begin{figure}[!t] 
\centering
\hspace{-25pt}
\includegraphics[width=0.88\linewidth]{fig/figSimFKNNErrorMap.jpg}\\
\caption{\TianModify{}{By visualizing the test-set error distribution, we quantified the discrepancy between $\mathcal{N}_{fk}$'s predictions and the simulator’s direct outputs, then highlighted the frame with the largest error.}}\label{fig:SimFKNNError}
\end{figure}

\subsubsection{FlexPAL}
\label{secFlexPAL}
\TianModify{}{As shown in Fig. \ref{fig:HardwareSystem}(d), the soft robot (FlexPAL) consists of three segments, each housing three soft-bellow actuators. Each actuator can deform both by inflating under positive pressure and by compressing under negative pressure. By adjusting the internal pressure of each actuator, FlexPAL can compress from its natural length of 92.0 cm down to 65.0 cm and also execute rotational deformations. The sim-to-real approach presented here accurately models FlexPAL’s entire external surface—information that is vital for ensuring collision-free motion planning.}





%


\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figSim2RealLearning.jpg}\\
\vspace{-5pt}
\caption{Result of different free-form surfaces predicted by our forward kinematics pipeline (i.e., Fig.\ref{fig:NNBasedFK} and Eq.(\ref{eqSim2RealPrediction})) while changing the actuation parameters (a). Four instants (A1-A4) are selected to apply onto the physical setup with the resultant shapes scanned and compared with the predicted shapes, where the shape approximation errors are visualized as colors.
The results with and without sim-to-real transfer (denoted by corrected and simulated models respectively) are compared in both the color maps (b) and the error histograms (c).
}\label{fig:Sim2RealEffectiveStudy}
\end{figure*}


\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figBaselineComp.png}\\
\vspace{-5pt}
\caption{Comparison of our function-prediction based sim-to-real method vs. the marker-prediction based method (as baseline). (Top) The errors between the scanned shape and the predicted shape when more and more frames of markers are employed for the sim-to-real learning. (Bottom) The scanned surface and the error maps of the predicted surfaces.
}\label{fig:Sim2RealComparison}
\end{figure}

\subsection{Details of Networks and Training}\label{subsecImplementationDetails}
For the training of forward kinematics network $\mathcal{N}_{fk}$, a dataset with 1,000 different pairs of actuation and shapes is collected from the simulation. This dataset contains shapes with the minimal and the maximal pressures applied to every chamber -- in total $2^k$ shapes were generated with $k$ being the DoFs of actuation (see Table \ref{tab:LearningData} shown parameters for different robots). We also randomly sampled other $(1000-2^k)$ actuation parameters using the Halton sequence \cite{halton1960efficiency}. All these 1,000 samples of actuation are applied in the simulation system to obtain their simulated shapes to explore the whole deformation space. Considering the large non-linearity between actuation and shape, we non-uniformly resample the actuation space by the amount of chamber inflation to enhance the training accuracy. The average time used for completing each simulation has been reported in Table \ref{tab:LearningData}. This dataset based on simulation is separated in the ratio of $7:3$ for training and testing.


We carefully select the network structure, which includes the number of hidden layers (\textit{h}), and the number of neurons in each hidden layer (\textit{l}). The experimental results of the maximal shape prediction error according to different network structures are studied and illustrated in Fig.~\ref{fig:NfkTraining}(a), and we choose two hidden layers with each layer contains 128 neurons as the final network structure to balance the quality of training result and the computational cost. In our implementation, ReLU is selected as the activation function and batch normalization is applied to improve stability in training. Note that our experiment finds that prediction with better quality can be achieved when learning the translation vectors applied to the positions of control points on an average model of all training shapes.




%D:\RepGeo\FullBody_IK\SoRo_NinethVersion\3-training\Train\TestingResult\code-calculateMesh2MeshError

%\revisionTian{The network $\mathcal{N}_{fk}$ is designed with two hidden layers, where each layer contains 128 neurons with ReLU as activation function.}{} \Tian{This part has been moved to the previous paragraph} As aforementioned, the input layer of $\mathcal{N}_{fk}$ contains the actuation parameters as a vector $\mathbf{a}\in\mathbb{R}^9$, and the output layer is the positions of $30 \times 30$ control points. \Tian{We might need to clearly state the rationale as reviewer requested.}\revisionTian{}{The reasons for choosing control points instead of vertices on the simulated mesh are that: 1) Its flexibility and efficiency in describing complex shapes with relatively fewer DoFs than mesh representation (around 10k vertices), which leads to efficiency in training; 2) It offers better parametric control in a sub-space, enabling easier manipulation and deformation of shapes, resulting in better training accuracy. As shown in Fig.\ref{fig:NfkTraining}(b), the average prediction error using control points representation was reduced $65.4\%$ on the test set, compared to that using mesh representation. It is also interesting to observe that prediction with even better quality can be achieved when learning the offsetting vectors applied to the positions of control points on an average model of all training shapes (just 0.27 mm).}

For the function prediction network $\mathcal{N}_{rbf}$ of sim-to-real transfer, we employ a network architecture with 2 hidden layers where each layer has a certain number of neurons using the ReLU activation function. The input layer contains the positions of $30 \times 30$ control points, and the output layer is the coefficients for the RBF-based warping function as $\bm{\gamma} \in \mathbb{R}^{3(N+4)}$ with $N$ being the number of \TianModify{kernals}{kernels}. The training of $\mathcal{N}_{rbf}$ is taken on 30 or 40 frames of markers obtained from either MoCap or scanner while randomly varying the pneumatic actuation within the working range of the chambers. Among these captured frames, a certain number of frames have missing markers. However, all captured markers (even for those from frames with missing markers) are employed as samples to train $\mathcal{N}_{rbf}$. The total number of valid markers for different cases have been reported in Table \ref{tab:LearningData}. Using the dataset of deformable mannequin generated from MoCap, it can be observed from the study as shown in Fig.~\ref{fig:NfkTraining}(b) that the prediction error starts to increase when the total number of neurons exceeds 50 -- i.e., overfitting happens. Based on this analysis, we select 24 neurons for each layer in $\mathcal{N}_{rbf}$. \TianModify{}{For the confidence network $\mathcal{N}_{conf}$, it takes the input vector includes simulated position (x,y,z) and the control points $\mathcal{S}^c(a)$ as global features. This combined input is propagated through three fully connected hidden layers—each containing 128 neurons and followed by a ReLU activation—and finally through a single-neuron fully connected layer with a Sigmoid activation, yielding a confidence score in the range $[0,1]$.}

% \begin{figure}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figNNStructureStudy.jpg}\\
% \caption{\rev{}{Study of network parameters \JENew{taken on the soft deformable mannequin} -- (a) the maximal shape prediction error w.r.t. different numbers of layers ($h$) and numbers of neurons per layer ($l$) are evaluated to choose the `best' values of $h$ and $l$ for $\mathcal{N}_{fk}$ (circled by black dash lines), and (b) the average shape prediction error w.r.t. the number of neurons in $\mathcal{N}_{rbf}$ is studied to avoid overfitting while training $\mathcal{N}_{s2r}$ using a limited number of samples. Note that $\mathcal{N}_{s2r}$ contains $\mathcal{N}_{rbf}$ plus a space warping module as illustrated in Fig.\ref{fig:comparisonSim2RealPipelines}.}}\label{fig:NfkTraining}
% \end{figure}
In our implementation, we first train $\mathcal{N}_{fk}$ and then train $\mathcal{N}_{rbf}$ \TianModify{}{and $\mathcal{N}_{conf}$}  by fixing $\mathcal{N}_{fk}$. The RBF-based space warping function $\mathbf{\Phi}$ and the B-spline shape decoder $\mathbf{B}$ are both implemented as differentiable layers, enabling seamless integration into the standard training process of $\mathcal{N}_{rbf}$. 
Having a surrogate model $\mathcal{N}_{fk}$ that is trained by physics-based simulation is essential to achieve satisfactory results of shape prediction.  \Tian{Put simulation v.s. predicted simulation distribution asked by reviewer 3}
\TianModify{}{The reasons are: (1) $\mathcal{N}_{fk}$ is built to replace the time-consuming simulator (similar to ref.~\cite{bern2020soft, Fang2022Sim2Real}) to achieve real-time computation while maintaining the accuracy as shown in Fig.\ref{fig:SimFKNNError}; (2) It provides valid backward gradients for IK computations, enabling iterative refinement of the actuation parameters.}

%As an alternative, researchers might directly train a network to predict the positions of markers $\{\mathbf{p}^*\}$ by $\mathbf{a}$ and then deform the rest shape of human body\charlie{robot?}\Tian{deformable mannequin} by the RBF-based warping function $\Phi(\cdot)$ \cite{Charlie2007RBFVolPara}. However, large shape approximation errors will be generated by this alternative without $\mathcal{N}_{fk}$ (see the middle \charlie{middle column?}\Tian{Yes.} of Fig.~\ref{fig:compFKLearning}(a)). The other interesting study is about the output of $\mathcal{N}_{fk}$. As can be observed from the comparison given in Fig.~\ref{fig:compFKLearning}(b), the B-spline surface representation used in our pipeline results in much smaller shape approximation error than directly predicting the positions of mesh vertices. The average shape approximate error is evaluated on each model of a test set with 300 individuals \charlie{individual bodies? have we discussed the CAESAR dataset before? figures?}\Tian{This is not the target human body from CAESAR dataset. It is the simulated deformed shape for sim FKNN}, and the distribution of errors among all individuals are plotted as a histogram to conduct the comparison. The mean of error distribution can be reduced from 1.82 mm to 0.63 mm \charlie{on the half size of mannequin model?}\Tian{After checking, Yes.} when learning B-spline control points instead of mesh vertices by $\mathcal{N}_{fk}$.
%\begin{figure}[t] \centering
%\includegraphics[width=1.0\linewidth]{fig/figDirectTrain_OurMethod.jpg}\\
%\caption{Study of different alternatives. (a) Much larger of shape approximation errors are generated by using an alternative method (without the simulation-based $\mathcal{N}_{fk}$ network) that first predicts the positions of markers from actuation and then deform the body shape by marker-based RBF deformation~\cite{Charlie2007RBFVolPara} -- see results shown in the middle column. (b) Comparison of the shape prediction errors (i.e., the average error of $18,000$ sample points on each model) among a test set with 300 individuals generated by $\mathcal{N}_{fk}$ when outputting the B-spline control points as compact shape descriptor (blue) vs. the mesh vertices (red).\Tian{This is to answer the question asked the reviewer's comments: "why so many networks are used?". Should we somehow remove this figure?}\charlie{to remove}
%}\label{fig:compFKLearning}
%\end{figure}


%\rev{}{In our pipeline, $\mathcal{N}_{fk}$ is working together with B-spline decoder $\mathbf{B}$ and gives a NN-based fast shape approximation to replace the time-consuming simulation process. Without $\mathcal{N}_{fk}$ as a prior, directly predicting the real surface suffers from sparse information and will generate an unsmoothed shape, as shown in the middle of Fig.~\ref{fig:compFKLearning}(a). We also compare the selection of shape representation when learning $\mathcal{N}_{fk}$. It can be seen from Fig.~\ref{fig:compFKLearning}(b) that the B-spline surface representation used in our pipeline gives a better training result - with $\mathcal{N}_{fk}$ training error reduced from 1.82 mm to 0.63 mm compared with direct learning with mesh vertices position. 
%Inviting B-spline representation also contributes to subsequent sim-to-real transfer with trained $\mathcal{N}_{rbf}$ and space warping function $\mathbf{\Phi}$, providing an efficient and robust correspondence in uv coordinates between data frame.} 

%Comparison experiments were conducted to evaluate the performance of the proposed method (b) against the naive learning approach (c), which directly learns from the actuator and the configuration space using captured markers. Following the training phase, both networks were assessed by calculating their error to a scanned model (a). The results clearly demonstrate that, although the naive method may achieve comparable error near the markers ($3.51$ mm v.s. $1.92$ mm), it fails to maintain the natural details in other areas ($7.43$ mm v.s. $1.38$ mm).

%\Tian{In Meta-Review: "reviewers request additional distinction of the various NN’s and more explanation of why several are necessary", we might need to explain why we need to learn $\mathcal{N}_{fk}$ first, why not directly learn act-surface mapping. We have conducted a comparison to directly learn actuation to marker position v.s. learn  $\mathcal{N}_{fk}$ +  $\mathcal{N}_{s2r}$}. \revisionTian{}{The reasons why we didn't directly learn the relationship between actuator space and configuration space of soft surfaces with only captured marker data are: 1) Generating a large and dense dataset in the physical setup is time-consuming and problematic; 2) The ground-truth data are sparse and even incomplete, leading to a reduced order of information on the shape of the free-form surface, can not preserve the fine-grained details of the massive regions between markers. On the contrary, our proposed method, first learned  $\mathcal{N}_{fk}$ in simulation, serving as prior during training  $\mathcal{N}_{s2r}$ (output fixed model $\mathcal{S}^*$) to better match with the physical shape $\mathcal{S}^{p}$. In this comparison study, the inputs of the naive learning network are the actuation parameters and the uv parameters of the query point, while the output is the point on the fixed model. The results are drawn in Fig.\ref{fig:DirectTrain_vs_OurMethod}, which clearly shows that near the marker regions, the average errors of the naive learning can achieve comparable prediction errors as our function-based learning ($3.51$ mm v.s. $1.92$ mm), but the whole surface shapes are chaos with no fine details with an average error of $7.43$ mm, which validates the importance of $\mathcal{N}_{fk}$ as training prior in our proposed method (average error is $1.38$ mm).}\Tian{provide experimental data and figure:To be done 08 04 2024; Finish drafting}

%For the RBF space warping function as shown in Fig.~\ref{fig:comparisonSim2RealPipelines}, we customize the forward and backward function in PyTorch to make it compatible as a differentiable layer, enabling seamless integration into the standard training process\Tian{add this}.
%\Tian{should we mention, we first train Nfk, then fix Nfk, train Nrbf?}





\subsection{Results of Sim-to-Real Learning by Motion Capture}\label{subsecResSim2RealSparse}
Experimental tests have been conducted to verify the performance of our sim-to-real method \JENew{with sparsely and partially acquired marker sets -- obtained by the motion capture system}. First of all, we randomly change all the nine actuation parameters of $\mathbf{a}$ and use our forward kinematic network to predict free-form surface shapes. Four instances are selected to apply the actuation $\mathbf{a}$ onto the physical setup. The resultant shapes on the soft robotic mannequin are scanned and compared with the simulated models (i.e., without sim-to-real transfer) and the corrected models (i.e., using the full pipeline with the sim-to-real network). The shape approximate errors are evaluated by first correcting the pose of scanned model using the ICP-based registration and then compute the distances between every surface sample points to their closest points on the scanned model. As can be found from the results shown in Fig.\ref{fig:Sim2RealEffectiveStudy}, the shape approximation errors on the corrected models were significantly reduced. The reductions are $30.4\%$, $53.5\%$, $32.1\%$ and $33.5\%$ for the average error and by $6.7\%$, $44.0\%$, $50.6\%$ and $60.6\%$ for the maximal error. 








% \begin{figure*}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figMembraneResult_RevisionExp.jpg}\\
% \vspace{-10pt}
% \caption{
% }\label{fig:sim2realOnMembraneRevision}
% \end{figure*}


% \begin{figure*}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figMembraneResult.jpg}\\
% \vspace{-10pt}
% \caption{
% \JENew{Shapes predicted by using simulation, direct learning and our $\mathcal{N}_{fk}+\mathcal{N}_{s2r}$ based pipeline are compared on the deformable membrane: (a) the average shape errors measured on 10 different randomly selected actuation configurations, (b) the histograms of shape error distributions on the configuration A1 and A2, and (c) the predicted shapes of the deformed membrane and their geometry errors displayed in colormap.
% } 
% \Tian{Add one figure after this figure to demonstrate the 400 training data}
% }\label{fig:sim2realOnMembrane}
% \end{figure*}

% \begin{figure*}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figMembraneResult_RevisionExp.jpg}\\
% \vspace{-10pt}
% \caption{
% }\label{fig:sim2realOnMembraneRevision}
% \end{figure*}

We then study the effectiveness of our function-prediction based sim-to-real pipeline by comparing it with the marker-prediction based pipeline as discussed in Sec.\ref{subsecRBFSpaceWarping}, where a trained network $\mathcal{N}_{mk}$ is employed to predict the positions of physical markers using the set of simulated marker positions and then determine the warping function for deformation. 
%A straightforward solution is to train a network $\mathcal{N}_{mk}$ to predict the positions of physical markers using the set of simulated marker positions as $\{ \mathbf{q}^* \}=\mathcal{N}_{mk}(\{ \mathbf{q} \})$. After that, the predicted positions of the physical markers and the positions of the virtual markers can be used to determine the value of $\bm{\gamma}$ and therefore also the warping function.
While randomly changing the pneumatic actuation, markers attached on the surface of the physical mannequin are progressively captured by the Vicon system and employed to train the sim-to-real networks. The trained networks are then employed to work together with $\mathcal{N}_{fk}$ to predict the free-form surfaces generated by a random selected actuation $\mathbf{a}_r$. The shape approximation errors are measured between the predicted shapes and the real surface, which is captured by scanning the physical model deformed by applying $\mathbf{a}_r$. The baseline method can only use those frames with full set captured markers for training. As shown in Fig.\ref{fig:Sim2RealComparison}, our method can predict a surface shape with smaller error. This mainly because that all captured markers can contribute to the sim-to-real training of our function-prediction based model even when they are on frames with missing markers. Differently, among all 40 frames involved in the tests shown in Fig.\ref{fig:Sim2RealComparison}, only about 55\% can be employed by the marker-prediction based method. The other 45\% frames all have 1 to 8 missing markers due to the occlusion caused by large deformation on chambers.



\subsection{Results of Co-learning the Function Space and Registration}\label{subsecResSim2RealDiffRegistration}

\TianModify{}{Training the proposed sim-to-real method with motion-capture data is straightforward and considerably simpler than with general point clouds, since frame-to-frame correspondences are already known during data acquisition with motion-capturing. However, when extending to a correspondence-free scanning setup, the lack of pointwise matches—i.e., for any simulated point, its counterpart in the scanned cloud is unknown (see Fig.~\ref{fig:motivation}(b))—poses a major challenge. Compounding this, missing regions in scans of deformable surfaces introduce further complexity. As such, some simulated points may have no valid targets at all, and, since the subset of missing correspondences evolves dynamically throughout training, it cannot be accurately determined in advance which points will lack matches, adding yet another layer of complexity.}


\TianModify{}{
In this section, the effectiveness of our co-learning architecture is validated by comparing it to sim-to-real learning with fixed correspondence, which is generated by the non-rigid registration algorithm \cite{yao2020quasi}.}

\TianModify{}{
As shown in Fig.~\ref{fig:coLearnDefCorrespondence}(a), the scan contains an incomplete region. Using precomputed correspondences \cite{yao2020quasi}, our corrected model deforms from the simulated shape to align with this scan. Although the deformation progressively matches the scanned surface, some areas remain unfilled. 
In contrast, our approach—illustrated in Fig.~\ref{fig:coLearnDefCorrespondence}(b)—employs a co-learning strategy coupled with a differentiable registration module to effectively resolve correspondence mismatches. The accompanying confidence-score colormap encodes the estimated reliability of each point’s match on the corrected model w.r.t. the scan. As training progresses, the vast majority of the surface transitions to dark blue—signifying high confidence—while only the scan’s missing regions remain red. Moreover, the zoomed inset demonstrates that our corrected model conforms precisely to the scanned geometry, unlike in Fig.~\ref{fig:coLearnDefCorrespondence}(a), where the corrected model protrudes beyond the intended surface.}


\TianModify{}{
To validate the robustness of our method, two different cases are plotted in Fig.~\ref{fig:coLearnDefCorrespondence}(c)\&(d). The intermediate values of the chamfer distance for these four cases are visualized in Fig.~\ref{fig:coLearnDefCorrespondence}(e), revealing that although the sim-to-real approach with fixed correspondences converges rapidly, the co-learning framework ultimately achieves significantly lower Chamfer distances.
}


\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figDiffReg.jpg}\\
\vspace{-0pt}
\caption{
\TianModify{}{Compared to the sim-to-real learning with fixed correspondence (a), the co-learning pipeline is capable of automatically updating the correspondence and confidence with the help of the differentiable registration module (b-d), which exhibits better convergence and tolerance to incomplete scan and large reality gap from the simulation.}
}\label{fig:coLearnDefCorrespondence}
\end{figure*}

\subsection{Results of Sim-to-Real Learning by 3D Scanning on Deformable Membrane}\label{subsecResSim2RealDense}
\begin{figure*}[!t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figMembraneResult.jpg}\\
\vspace{-0pt}
\caption{
\JENew{Shapes predicted by using simulation, direct learning and our $\mathcal{N}_{fk}+\mathcal{N}_{s2r}$ based pipeline are compared on the deformable membrane: (a) the average shape errors measured on 10 different randomly selected actuation configurations, (b) the histograms of shape error distributions on the configuration A1 and A2, and (c) the predicted shapes of the deformed membrane and their geometry errors displayed in colormap.
} 
}\label{fig:sim2realOnMembrane}
\end{figure*}
\begin{figure}[!t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figMembraneResult_RevisionExp.jpg}\\
\vspace{-5pt}
\caption{To further assess the transfer efficiency of our approach versus the direct learning baseline, we collected a larger dataset of 500 frames—400 for training and 100 for testing. Under identical training conditions, our method delivers substantially better performance.
}\label{fig:sim2realOnMembraneRevision}

\end{figure}


\JENew{After studying the effectiveness of our sim-to-real approach on sparse information obtained from a motion capture, we study its performance on dense input as 3D point clouds. The proposed sim-to-real approach was applied to the deformable membrane, using a structure-light-based scanner to capture data for training and testing. Ten randomly generated unseen actuation parameters were applied to the physical hardware, and the corresponding shapes are predicted by our $\mathcal{N}_{fk}$ and $\mathcal{N}_{s2r}$ networks and compared with the scanned shape. The results of the comparison are shown in Fig.\ref{fig:sim2realOnMembrane}, where the geometric errors are visualized on surfaces by colormaps, and the statistical error distributions are given as histograms. For the two selected configurations -- A1 and A2, the average errors have been reduced by 75.5\% and 63.3\% with the maximal errors reduced by 41.8\% and 58.6\% accordingly. 
}
%\TianModify{}{To validate the generality of our method,  As shown in Fig. \ref{fig:sim2realOnMembrane}(a), Ten randomly generated unseen actuation parameters were applied to the physical setup, and the corresponding shapes (labeled as "Scanned Model") were reconstructed in Fig. \ref{fig:sim2realOnMembrane}(c). These shapes were then compared with both the simulation model and a corrected model to calculate shape errors, which are visualized as error colormaps in Fig. \ref{fig:sim2realOnMembrane}(c), with four frames selected for detailed analysis. The error distribution is further illustrated in Fig. \ref{fig:sim2realOnMembrane}(b). Notably, our method successfully captures the reality gap across a sequence of different shapes. The average and maximum errors for these distributions are presented in Fig. \ref{fig:sim2realOnMembrane}(a) to provide an overview. For cases A–D, the average error was reduced by 75.5\%, 73.9\%, 63.3\%, and 74.0\%, respectively, while the maximum error decreased by 41.8\%, 53.4\%, 58.6\%, and 45.4\%.}

\subsubsection{Why not directly learn from physical experiment}
\JENew{
After taking the above study and comparison, we are also curious what if we directly learn the shape from the actuation parameters as input using neural networks. We applied 40 random actuations to the deformable membrane and record the corresponding physically deformed shapes as the training dataset. The direct learning network consists of two hidden MLP layers with 128 neurons in each layer. The input of the network is actuation parameters (i.e., 9 values for each shape) and the output is 200 points sampled on the deformed surface. Hausdorff distance \cite{HausdorffLossTorch} and chamfer distance \cite{ChamferLossTorch} are jointly used to reduce both maximum and average errors between two point clouds, with weights of 1.0 and 5.0, respectively. Lipschitz loss\cite{liu2022learning} is utilized to penalize the Jacobian magnitude of trained neural network. The resultant surfaces of prediction are then generated by RBF-based surface deformation using these 200 predicted sample points. The comparison between this direct learning method and our $\mathcal{N}_{fk}$ and $\mathcal{N}_{s2r}$ networks-based prediction has also been given in Fig.\ref{fig:sim2realOnMembrane}. Direct learning leads to results with significantly larger errors.
}

\TianModify{}{To further evaluate the effectiveness of our sim-to-real learning method against the direct learning approach, we collected a dataset of 500 frames—400 for training and 100 for testing. We then trained both models in parallel and plotted their average error on the test set.}

\TianModify{}{In Fig.\ref{fig:sim2realOnMembraneRevision}(a), our sim-to-real approach yields substantially lower error than direct learning when using the same number of training frames—2.27 mm versus 4.02 mm with 40 frames. As more frames are added, both methods see improved accuracy. Crucially, the direct learning method requires 400 frames to reach a 2.29 mm error, matching the 2.27 mm achieved by our method with only 40 frames, which underscores the transfer efficiency gained from leveraging simulation priors and RBF-space warping. When trained on the full set of frames, our sim-to-real model further reduces the average error to 1.95 mm. The detailed error distributions are shown in Fig.\ref{fig:sim2realOnMembraneRevision}(b).} 

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figFrequencyDistribution.jpg}\\
\vspace{-10pt}
\caption{\Remove{Frequency spectrum of the shape approximation error reduced by our sim-to-real method for the A1 shape shown in Fig.\ref{fig:sim2realOnMembrane} is given in (a) and compared with the frequency spectrum of white noise (b).}\Tian{considering remove this figure according to reviewer 3}
}\label{fig:FrequencyAnalysis}
\end{figure}
\subsubsection{Frequency analysis of sim-to-real errors} 
\Remove{The reduction in sim-to-real error achieved by our method is computed as the difference between the shape error of the simulated model and that of the corrected model, which can be represented as a height field for the deformable membrane. We use the Fast Fourier Transform (FFT)} \cite{duhamel1990fast} \Remove{to analyze the frequency spectrum of these reduced errors as shown in Fig.\ref{fig:FrequencyAnalysis}(a) for the A1 shape in Fig.\ref{fig:sim2realOnMembrane}.
Compared to the frequency spectrum of white noise (Fig.\ref{fig:FrequencyAnalysis}(b)), our method’s error reduction primarily falls within the low-frequency band. This also explains why we can effectively reduce the error by a relative small number of samples for training the $\mathcal{N}_{s2r}$ network.}\Tian{suggested by reviewer 3}




%\TianModify{}{Frequency analysis is conducted by applying the Fast Fourier Transform (FFT \cite{duhamel1990fast}) to the reduced error on deformable membrane setup, which is calculated as the difference between the shape error of the corrected model (from our Sim-to-Real method) and the shape errors of the simulation model for the Case A in Fig.\ref{fig:sim2realOnMembrane}. The results show the reduced error is primarily concentrated in the low-frequency domain (shown in Fig. \ref{fig:FrequencyAnalysis}(a)) compared to the frequency spectrum of white noise (shown in Fig. \ref{fig:FrequencyAnalysis}(b)), which indicate that our Sim-to-Real method is mainly adjusting the low-frequency distortion of the simulation model.}

%\begin{figure}[t] 
%\includegraphics[width=1.0\linewidth]{fig/figDirectLearning.jpg}\\
%\caption{\TianModify{}{Shape error distribution in two unseen cases: (a) In the first case, for the direct learning method, the maximum error is 21.16 mm and the average error is 4.26 mm; For our method, the maximum error is 6.43 mm and the average error is 1.42 mm; (b) While in the second case, for the direct learning method, the maximum error is 14.96 mm and the average error is 5.17 mm; For our method, the maximum error is 6.48 mm and the average error is 1.81 mm.}\Tian{Add Real Photos -- Membrane}
%}\label{fig:DirectLearning}
%\end{figure}

% \begin{figure}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figDirectLearning.jpg}\\
% \vspace{-10pt}
% \caption{ 
% \TianModify{}{Shape error distribution in two unseen cases: (a) In the first case, for the direct learning method, the maximum error is 21.16 mm and the average error is 4.26 mm; For our method, the maximum error is 6.43 mm and the average error is 1.42 mm; (b) While in the second case, for the direct learning method, the maximum error is 14.96 mm and the average error is 5.17 mm; For our method, the maximum error is 6.48 mm and the average error is 1.81 mm.}
% }\label{fig:DirectLearning}
% \end{figure}

% \begin{figure}[t] 
% \centering
% \vspace{-10pt}
% \includegraphics[width=1.0\linewidth]{fig/figFrequencyDistribution.jpg}\\
% \vspace{-10pt}
% \caption{ 
% \TianModify{}{Frequency Analysis.}
% }\label{fig:FrequencyAnalysis}
% \end{figure}


%\begin{figure}[t] \centering
%\includegraphics[width=0.9\linewidth]{fig/figSimSparseDenseComp.jpg}\\
%\caption{ \TianModify{}{When applying the same unseen actuation parameters, the prediction error of the simulation model and two types of corrected models are drawn in (a), and the distributions are further plotted in (b) for comparison.}
%}\label{fig:SimSparseDenseComp}
%\end{figure}
%
%\TianModify{}{with the randomly generated actuation parameters (same as in Sec.\ref{subsecResSim2RealSparse}) applied on the deformable mannequin setup, the 3D scanner is used to capture the deformed geometries of the free-form surfaces as point cloud, followed by pre-processing steps to generate correspondence for training, as indicated in Sec.\ref{secSim2RealwithDenseInput}.}
%
%\TianModify{}{Then, the unseen actuation parameters are applied to generate a scan model (acquired from 3D scanning), simulation model, corrected model (trained on sparse information), and corrected model (trained on dense information). The shape error of the simulation model and two types of corrected models are visualized in Fig.\ref{fig:SimSparseDenseComp}(a), which clearly shows the corrected model trained on a dataset consisting of sparse information can already achieve error reduction. It is especially encouraging that our Sim-to-Real method can more accurately bridge the reality gap across the entire surface domain, thanks to the dense information (here are 500 sample points for each scan) in the training set. The error distribution is illustrated in Fig.\ref{fig:SimSparseDenseComp}(b). Note that the average error of the corrected model (from dense info.) is 2.16 mm, which is 20.2\% lower than the corrected model trained from sparse information (2.71 mm).}

\begin{figure}[t] 
\centering
\vspace{-10pt}
\includegraphics[width=1.0\linewidth]{fig/figSamplePntDensity.jpg}\\
\vspace{-5pt}
\caption{\JENew{Experimental tests to study the accuracy of shape prediction (a) when using different number of `virtual' markers for the sim-to-real learning. (b) The results in terms of average geometric errors are compared with the sim-to-real result by using 34 real markers.}
}\label{fig:SamplePntDensityStudy}
\end{figure}

\begin{figure}[t] 
\vspace{-5pt}
\centering
\includegraphics[width=1.0\linewidth]{fig/figKernelNum.jpg}\\
\vspace{-5pt}
\caption{\JENew{The experiment demonstrates how the number of RBF kernels affects the accuracy of prediction (measured as the average of shape approximation error) and the computational cost (measured as the required time to evaluate $10^5$ warping operations. Four different shapes (as A1-A4 shown in Fig.\ref{fig:Sim2RealEffectiveStudy}) are evaluated in this tests.}
}\label{fig:DiffKernelNum}
\end{figure}

\subsection{Number of `Virtual' Markers and Kernels} 
\JENew{When conducting sim-to-real learning with dense point cloud input, selecting an appropriate number of `virtual' markers is essential. We generated datasets with varying numbers of virtual markers to train the sim-to-real network $\mathcal{N}_{s2r}$. After training, these networks were tested on unseen cases to evaluate the accuracy of shape prediction. As shown in Fig.\ref{fig:SamplePntDensityStudy}(a), the approximation error decreases while the number of virtual markers increases, stabilizing after approximately 500 markers. When compared to networks trained on sparse but real markers, the corrected models trained with the same number of real markers outperform those trained with virtual markers (see Fig.\ref{fig:SamplePntDensityStudy}(b)). This may be due to the fact that motion capture datasets offer accurate correspondence, whereas datasets from 3D scans introduce inaccuracy due to registration errors.}

%\subsection{Number of Kernels}
%\input{tex/TabDifferentKernels}
\JENew{The number of Gaussian kernels, denoted as $N$ in Eq.\eqref{eqRBFSpaceWarping}, is also a factor influencing the accuracy and efficiency of the sim-to-real method. With too few kernels, the space warping function lacks the capacity to capture complex variations, leading to notable errors. Conversely, an excessive number of kernels increases computational demands, heavily impacting the IK computation as it must repeatedly apply the RBF-based space warping. To determine the number of kernels, we maintain 500 virtual markers and train different sim-to-real networks on the same dataset, varying only the number of kernels. Shape approximation errors were then evaluated on four unseen cases, with results shown in Fig.\ref{fig:DiffKernelNum}. As a result, more kernels generally lead to higher prediction accuracy but at the cost of longer computation times. To balance between the accuracy and the efficiency, we select 100 kernels for our implementation and tests.}

\subsection{Generality to Handle Compression Deformation} 

\begin{figure}[t] 
\vspace{-5pt}
\centering
\includegraphics[width=1.0\linewidth]{fig/figCompression.jpg}\\
\vspace{-5pt}
\caption{\TianModify{}{(a) The experiment aims to validate the generality of our sim-to-real method in modeling the robot's outer surface (FlexPAL) with compression deformation. In comparison to the simulated model, the function-based sim-to-real method significantly reduces the reality gap, with the error distribution shown in (b). Three distinct states are extracted and displayed in (c).}}
\label{fig:Compression}
\end{figure}

\TianModify{}{To validate the effectiveness of our method in accurately handling the sim-to-real deformation modeling of the robot ("FlexPAL") with compression deformation, we have collected a simulation dataset using Mujucoo and a corresponding real dataset from the physical setup. As illustrated in Fig.\ref{fig:Compression}(a), the outer surface enclosing the body of FlexPAL is designated as the target for modeling. For the real dataset, we collected 700 samples, with 500 allocated for training and 200 for testing. The proposed sim-to-real method demonstrates significantly improved accuracy on the test set, as shown in Fig.\ref{fig:Compression}(b). Furthermore, in Fig.\ref{fig:Compression}(c), three frames from the testing set (in original state, compressed state, and rotated state, respectively) are visualized with the simulated model, corrected model, and the ground-truth are drawn together to show the difference.}

\subsection{Effectiveness of Compatibility Loss} 
\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figCompatibleComp.jpg}\\
\vspace{-5pt}
\caption{ 
\JENew{An ablation study was conducted to test the effectiveness of the compatibility loss in sim-to-real learning based on two different simulators -- I: the one based on FEA~\cite{xavier2021finite} and II: the geometry-based simulator (ref.~\cite{Guoxin2020TRO,Guoxin2022IROS}), where both simulators are struggling to predict the deformed surfaces accurately (see (a)). It can be observed from the colormaps in (a) and also the histograms of distance errors and normal errors in (b) that the corrected model incorporating compatibility loss (labeled as `with C. Loss') produces a significantly improved shape comparing to the corrected model without compatibility loss (labeled as `without C Loss'). The generality of our approach has been proved as the sim-to-real gap can be effectively fixed on results generated by both simulators.}
}\label{fig:CompatibleCompare}
\end{figure*}

\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figIK_Membrane.jpg}\\
\vspace{-5pt}
\caption{\JENew{To verify the effectiveness of our sim-to-real approach for improving the accuracy of IK computation, experiments were conducted to deform the membrane into target shapes using the actuation parameters determined by IK with vs. without sim-to-real. The deformable membrane is employed as a reconfigurable mold for curved 3D printing in this example -- see (a) for the hardware setup consists of a UR10e robot arm equipped with a Pulsar™ Pellet Extruder. The tests are conducted for printing models on two different target shapes as shown in (b) and (d). The resultant shapes on the deformable membrane by IK with (bottom row) and without (top row) sim-to-real are given in (b) and (d) together with the color maps illustrating the shape approximation errors, where large approximation errors lead to large gaps between the printer head and the mold as indicated by the red arrows. In the top row of (c) and (e), we can find poor printing results caused by large gaps when sim-to-real is not applied. The gap can be significantly reduced after applying our sim-to-real approach -- see the improved results shown in the bottom row of (c) and (e).}
%\charlie{figure to be updated (14/12)}\Tian{Figure updated}
}\label{fig:IKResultMembrane}
\end{figure*}

\JENew{An ablation study was conducted on the soft manipulator setup to illustrate the importance of compatibility loss in achieving accurate shapes and reducing the gap between simulation and reality. This setup is selected due to its complex deformation, where both the global structure shape and the local surface shape are significantly changed. To further validate the effectiveness and the generality of our sim-to-real pipeline with compatibility loss, we have tested it by using two different simulators -- one is based on FEA~\cite{xavier2021finite} and the other is based on the geometry-based simulator (ref.~\cite{Guoxin2020TRO,Guoxin2022IROS}). The results can be found in Fig.\ref{fig:CompatibleCompare}. The normal error at any point $\mathbf{p}_j$ on a simulated (or corrected) surface is defined as:
\begin{equation}\label{eqNormalVarHistogram}
    \eta(\mathbf{p}_j) = 1-\mathbf{n}(\mathbf{p}_j) \cdot \mathbf{n}(\mathbf{c}^{\mathcal{T}}_j)
\end{equation}
with $\mathbf{c}^{\mathcal{T}}_j$ being the closest point of $\mathbf{p}_j$ on the scanned point cloud. The distribution of the distance errors and the normal difference errors are plotted as the histograms shown in Fig.\ref{fig:CompatibleCompare}(b). Note that the histograms of normal errors are capped at 0.06, according to an angular difference of less than $20^\circ$ between the two normals. This allows to zoom-into a range of interest for better comparison.}

%\TianModify{}{The proposed Sim-to-Real method is firstly applied on the simulator I, which comes from FEA with hyper-elastic material property from \cite{xavier2021finite}, and the corresponding experimental results are shown in Fig.\ref{fig:CompatibleCompare}(a), demonstrating the simulation ability to captures the the global structure shape, but still can not fully capture the local deformation (i.e., local inflation deformation) as shown from the colormap with an average error of 11.15 mm. Conversely, the corrected model from the proposed sim-to-real method (without compatible loss) can help improve the modeling accuracy (average error of 3.00 mm and maximum error of 17.54 mm), but it is still not ideal in the red areas indicated by the black dash line, which comes from the fact that the learned mapping is not compatible without the compatibility loss. As such, the corrected model trained with compatibility loss can mitigate this effect and ensure smooth space warping mapping can be learned during training (achieving an average error of 1.99 mm and maximum error of 12.37 mm). To further evaluate the surface detail matching, orientation accuracy is defined to calculate the normal difference between the two models and further being plotted in Fig.\ref{fig:CompatibleCompare}(b). Specifically, for any point $\mathbf{p}_j$ on the corrected model, calculate its normal difference $\eta(\mathbf{p}_j)$ defined as follows:}
%
%\TianModify{}{
% \begin{equation}\label{eqNormalVarHistogram}
%    \eta(\mathbf{p}_j) = 1-\mathbf{n}(\mathbf{p}_j) \cdot \mathbf{n}(\mathbf{c}^{\mathcal{T}}_j)
%\end{equation}}
%
%\TianModify{}{with $\mathbf{c}^{\mathcal{T}}_j$ being the closest point of $\mathbf{p}_j$ on the scanned model $\mathcal{T}$. After this operation, the greater the deviation, the closer $\eta(\mathbf{p}_j)$ approaches 1. Conversely, as the deviation decreases, $\eta(\mathbf{p}_j)$ tends to approach 0. The distribution of the distance error and normal difference error have been collected and plotted in  Fig.\ref{fig:CompatibleCompare}. It is important to note that the maximum normal error is capped at 0.134, corresponding to an angular difference of less than 30 degrees between the two normals. This cap allows us to zoom in on the specific range of interest for better illustration.}
%
%\TianModify{}{To prove the generality of our proposed sim-to-real method, it is then applied to reduce the sim-to-real gap for the geometry-based simulator~\cite{Guoxin2020TRO,Guoxin2022IROS}. As shown in Fig.\ref{fig:CompatibleCompare}(a), the simulator is able to produce the large local deformation but falls short in capturing the global curve shape of the manipulator, which, however, can be accurately compensated by the network, especially with the compatibility loss. The results of distance error and normal error distribution are provided to support the advantages.}

\JENew{The experimental tests shown in Fig.\ref{fig:CompatibleCompare} demonstrate that the compatibility loss is essential for achieving better shape accuracy on corrected models. They also confirm the generality of our network when working on different types of numerical simulators.}

%\subsubsection{Sim-to-Real from Different Simulation Frameworks} 
%\TianModify{}{To demonstrate the generality of our Sim-to-Real method in handling different simulation frameworks with varying levels of accuracy, two distinct simulation methods were selected and adapted using our Sim-to-Real approach.}
%\TianModify{TO FILL EXPERIMENTS}{}

% \begin{figure}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figProgressiveResult.jpg}
% \caption{The progressive results by applying our NN-based fast IK solver, where the curve shows the average shape approximation errors during the iterations of gradient descent. Using the actuation determined by our fast IK solver, a shape similar to the target model can be realized on the soft mannequin where the error analysis is conducted by 3D scanning with its result shown as the color map.
% }\label{fig:progressIKResult}
% \end{figure}

% \begin{figure}[t] 
% \centering
% \includegraphics[width=1.0\linewidth]{fig/figIKResults.jpg}\\
% %\vspace{-5pt}
% \caption{The physical results of our fast IK solver for three different target models, where the distributions of shape approximation errors are generated by scanning and visualized as the color maps. 
% }\label{fig:IKResults}
% \end{figure}

\subsection{Results of Inverse Kinematics}\label{subsecResIK}
\JENew{Our sim-to-real approach can enhance the precision of actuation parameters generated by the IK algorithm introduced in Sec.\ref{subsecGradientBasedIK}, enabling more accurate realization of the target shape. To validate the effectiveness of this approach, we conducted physical experiments on three soft robots to demonstrate its performance through examples of IK computation, including shape approximation on a deformable membrane to serve as a reconfigurable mold for curved 3D printing, motion planning of a soft manipulator with the help of swept volume computation and shape approximation on a deformable robotic mannequin.} 
%\Guoxin{the key is to define the target shape for the task of conformal printing as well as collision-free trajectory following - discussed with Yingjun on 11-01-2024}
%\Tian{IK for soft manipulator is added; IK for soft membrane is added 26-11-2024.}

\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figIK_Manipulator.jpg}
%\vspace{-5pt}
\caption{\JENew{This example demonstrates the importance of sim-to-real in motion planning to compute a collision-free trajectory for deforming the soft manipulator to touch the target ball while presenting a stick obstacle around -- see (a) for the models in simulation and reality. When using the kinematic computation without sim-to-real, the swept volume of a planned trajectory is as shown in (b). This trajectory however leads to collision when being applied to the physical setup (see the scanned results as shown in the left of (c)) due to the large gap between simulation and reality (see the right of (c)). Differently, when incorporating our sim-to-real approach into the kinematic computation, the planned trajectory is as given in (d) with its real execution results as scanned swept volume shown in the left of (e). The motion is collision-free in reality by benefiting from the accurate deformation prediction as illustrated in the right of (e).}
}\label{fig:IKResultManipulator}
\end{figure*}
 
\subsubsection{\JENew{Shape Approximation on Deformable Membrane}}
\JENew{The deformation of the soft membrane can be programmed into different shapes, enabling it to function as a reconfigurable mold for 3D printing. The hardware setup of our 3D printing experiment is as shown in Fig.\ref{fig:IKResultMembrane}(a), where the task of 3D printing is conducted by a UR10e robot arm~\cite{UR10e} equipped with a Pulsar$^\mathrm{TM}$ pellet extruder~\cite{Pulsar}. The material deposition printing process is conducted by following a toolpath computed on a surface. When the membrane can be accurately deformed into the target shape of this surface, the robotic hardware can print \textit{Polylactic Acid} (PLA) directly on this curved surface.}

\JENew{This application requires accurate shape control of the mold. For example, as shown in the top row of Fig.\ref{fig:IKResultMembrane}(b) and (d) circled by red dashed lines, there are large gaps between the printer head and the mold in the regions with large shape approximation errors (indicated by red arrows). Apparently, this will lead to inaccurate material deposition that results in poor shape control of 3D printed models -- see the top row of Fig.\ref{fig:IKResultMembrane}(c) and (e) around the regions indicated by red arrows where misalignment between two layers caused by the shape error of mold can be found. The shape errors can be significantly reduced after incorporating our sim-to-real method in the IK computation loop. The results with sim-to-real are given in the bottom row of Fig.\ref{fig:IKResultMembrane}(b-e) circled by blue dashed lines, where precise deposition of materials at the turning points can be achieved in 3D printing -- i.e., less misalignment is observed.
}

%The tests are conducted for printing models on two different surfaces as target shapes shown in (b) and (d). The resultant shapes on the deformable membrane by IK with (bottom) and without (top) sim-to-real are given in (b) and (d) together with the color maps illustrating the shape approximation errors, where large approximation errors lead to large gaps between the printer head and the mold as indicated by the red arrows. In the top row of (c) and (e), we can find poor printing results caused by large gaps when sim-to-real is not applied. The gap can be well fixed after applying our sim-to-real approach -- see the improved printing results shown in the bottom row of (c) and (e).

%\TianModify{}{In the scenario depicted in Fig.\ref{fig:IKResultMembrane}(b), a single target shape is provided to our IK solver, which determines the optimal actuation parameters to generate the predicted shape. Ensuring that the predicted shape of the deformable membrane closely matches the target shape is crucial, as the tool path for material deposition is pre-computed based on the predicted configuration. In this case, the toolpath with a flower pattern is generated. Without the Sim-to-Real approach, the IK solver produces a predicted surface with significant errors, leading to a large stand-off distance (SOD) when running the generated toolpath, where the extruded material is too far from the target shape. However, incorporating Sim-to-Real into the computation ensures an appropriate SOD. This marked improvement in accurately approximating the target shape significantly impacts the printing quality of the models shown in Fig.\ref{fig:IKResultMembrane}(c). The printed model without Sim-to-Real struggles with toolpaths involving sharp turns, whereas those utilizing Sim-to-Real handle these complexities effectively. A similar phenomenon can be observed in the second case, where a toolpath featuring Hilbert curve patterns is both generated and executed with/without Sim-to-Real in Fig.\ref{fig:IKResultMembrane}(d)\&(e).}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figProgressiveResult.jpg}
\caption{The progressive results by applying our NN-based fast IK solver, where the curve shows the average shape approximation errors during the iterations of gradient descent. Using the actuation determined by our fast IK solver, a shape similar to the target model can be realized on the soft mannequin where the error analysis is conducted by 3D scanning with its result shown as the color map.
}\label{fig:progressIKResult}
\end{figure}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figIKResults.jpg}\\
%\vspace{-5pt}
\caption{The physical results of our fast IK solver for three different target models, where the distributions of shape approximation errors are generated by scanning and visualized as the color maps. 
}\label{fig:IKResults}
\end{figure}


\subsubsection{\JENew{Motion Planning of Soft Manipulator}}
\JENew{The accurate shape prediction in kinematic computation is important for the motion planning of a soft robot. We conducted the physical experiment on a soft manipulator with 6 DoFs as shown in Fig.\ref{fig:IKResultManipulator}. Specifically, a sampling-based motion planning algorithm \cite{karaman2011sampling} is employed to compute a sequence of samples as actuation parameters that progressively deform the soft manipulator to touch the target ball while presenting an obstacle stick around the manipulator -- see Fig.\ref{fig:IKResultManipulator}(a) for the illustration. Without the sim-to-real correction, the shapes predicted by the kinematic computation are significantly different from the reality. This leads to a risk of collision on a planned collision-free trajectory (see Fig.\ref{fig:IKResultManipulator}(b) for the planned collision-free swept volume and Fig.\ref{fig:IKResultManipulator}(c) for the scanned models colliding with the obstacle stick). The problem can be well solved after incorporating our sim-to-real method into the kinematic computation -- see the results given in Fig.\ref{fig:IKResultManipulator}(d) and (e).}

%\charlie{Above edited; Working in this paragraph now (29/11)}
%
%\TianModify{}{The soft manipulator presented in this paper utilizes pneumatic actuators with 6 DoFs and features a highly deformable outer surface. In environments with obstacles, the manipulator's forward kinematics cannot be simplified through an analytical model that only captures its structural shape. Instead, accurate modeling of the configuration space, encompassing the entire outer surface, is required. Consequently, the swept volume of the planned trajectory must also be considered as a target for the soft manipulator to approximate.}

%\TianModify{}{In this experiment, illustrated in Fig. \ref{fig:IKResultManipulator}(a), the manipulator reaches toward a target ball while avoiding an obstacle. To ensure the entire manipulator remains collision-free, the swept volume of its planned trajectory is computed, as shown in Fig. \ref{fig:IKResultManipulator}(b), and defined as a series of target shapes for our IK solver. Without Sim-to-Real adjustments, depicted in Fig. \ref{fig:IKResultManipulator}(c), the scanned swept volume collides with the obstacle, showing significant geometric error relative to the planned trajectory, as highlighted by the colormap. In contrast, with Sim-to-Real integration, the IK solver enables the manipulator to reach the target without collision, as shown in Fig. \ref{fig:IKResultManipulator}(d), where the obstacle lies outside the solid of the scanned swept volume. These results demonstrate that the Sim-to-Real model provides a more accurate shape prediction, closely aligning with both the scanned model and physical outcomes.}



% \TianModify{}{In this experiment, the target location $\mathbf{p}^{t}$ is chosen to be reached by the specific point of the manipulator (its parameter is denoted as $(u_p,v_p)$), which can be written as Eq.\ref{eqSim2RealPrediction}: $\mathbf{p}^*(\mathbf{a},u_p,v_p)=\mathcal{N}_{s2r}(\mathbf{B}(u_p,v_p,\mathcal{S}^c(\mathbf{a})),\mathcal{S}^c(\mathbf{a}),\{ \mathbf{B}(u_q,v_q,\mathcal{S}^c(\mathbf{a})\})$ while the body $\mathcal{M}$ should be collision-free with obstacle $\mathcal{O}_{obs}$. Sampling-based method is used to generate feasible trajectories from the initial position to the target position while the predicted shapes are generated by our sim-to-real method. This can be formulated as an optimization problem:}


% \begin{align}
% \arg \min_{\mathcal{A}} & \sum_{t=1}^{n-1}  \| \mathbf{p}^*(\mathbf{a}_t,u_p,v_p)-\mathbf{p}^*(\mathbf{a}_{t+1},u_p,v_p)\|^2\label{eq:objective1}\\& \quad +\omega  
% \|(\mathbf{a}_{n},u_p,v_p) - \mathbf{p}^{t} \|^2 \label{eq:objective2}\\
% s.t. &  \quad \mathcal{M} \cap \mathcal{O}_{obs} = \emptyset\\
% & \quad \mathbf{a}_{min} < \mathbf{a} < \mathbf{a}_{max}
% \label{eq:targetReaching}
% \end{align}
% \Tian{Remove this equation}
% \TianModify{}{In this optimization problem, Eq.\ref{eq:objective1} is employed to maintain smooth transitions between neighboring waypoints, preventing abrupt changes, while Eq.\ref{eq:objective2} ensures that the target position is accurately reached.}

% \TianModify{}{Upon implementing the calculated trajectory on the robot, as depicted in Fig.\ref{}, the robot follows a smooth path to the target location, effectively maintaining obstacle avoidance for its deformed body throughout the movement.}


\begin{figure*}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figGarmentFab.jpg}\\
\vspace{-5pt}
\caption{\JENew{Sustainable and customized garment can be fabricated by using the deformable mannequin as a mold: (a) the mannequin is first deformed into the body scanned shape of a customer, (b) biodegradable material is placed on top of the mannequin and heated under a controlled temperature, (c) a mycelium layer is formed as a piece of garment in the mannequin's shape after heating, (d) the garment is taken off from the mannequin, and (e) the resultant  garment in a customized shape.}
}\label{fig:GarmentFabrication}
\end{figure*}

\subsubsection{Shape Approximation on Deformable Mannequin}
We have tested the performance of our NN-based fast IK solver on a variety of individual shapes presented in the CAESAR dataset. Figure \ref{fig:progressIKResult} shows the progressive results when applying our IK solver to realize the target shape on the physical setup of pneumatic driven deformable mannequin. It can be observed that our method converges very fast -- i.e., around 15 iterations where each iteration takes less then 0.5 second. 
%\Guoxin{The convergence speed is not the contribution of this work, and the IK solver is not presented in detail. what about also mention the time for single iteration here?} \charlie{I think we need to mention both.}
The distribution of shape approximation errors are generated by scanning the soft mannequin that has been deformed using the resultant actuation determined by our IK solver. \JENew{Results on three different models are given in Fig.\ref{fig:IKResults}}.

The effectiveness of our fast IK solver has been tested on other models randomly selected from the CAESAR dataset -- see the results shown in Appendix C. It can be find that the shapes realized on the robotic deformable mannequin can well mimic the shape of target models. This can also be verified by the quantitative analysis results generated by the 3D scanner.


% \Tian{All the following items should be removed}
% \subsubsection{\rev{}{Computational efficiency}}
% In this work, the NN-based IK computing pipeline enables fast and robust shape approximation for a deformable free-form surface. We have achieved a computing speed of less than 10 seconds per target model, which is significantly faster than existing methods and aligns well with the physical actuation time of the proposed setup. 
% \rev{}{The computational complexity of our pipeline is influenced by various factors, including the network architecture, the number of control points on the B-spline surface, and the kernel number of the RBF morphing function. The current selection is mainly based on experimental tests to find the balance between performance and efficiency. We can further accelerate the computation by GPU-based parallel computing.}

% \subsubsection{\rev{}{Applicability to other deformable robots}}
% \rev{}{Our pipeline is also applicable to other soft and deformable robotic systems. In principle, our function based sim-to-real learning method can be applied to a variety of deformable robots when their freeform shapes can be represented by B-spline surfaces (e.g., Chen \textit{et al.}~\cite{chen2023morphological}). We will further explore the potential of our method in other robotic setups, particularly for addressing data collection challenges with learning-based solutions.}
% %Thanks to the usage of effective B-spline based shape encoding in our framework, the complexity of network learning and kinematics computing remains less affected.

% \subsubsection{\rev{}{Different setups for data acquisition}}
% In this work, a well-calibrated motion capture system (with position tracking error less than 0.1 mm \cite{viconAccuracy}) is applied to capture data from the physical setup. 
% \rev{}{While our pipeline is designed for sparse yet accurate data from motion capture, it has the potential to be extended to cover the systems with LiDAR~\cite{LidarCamIntel} or RGBD cameras~\cite{IntelD457Camera, kurillo2022evaluating} that capture dense but less accurate point clouds.}
% %\rev{}{However, point cloud-based systems generally exhibit significantly higher noise levels than motion capture systems, and they cannot provide a good parameterization between data frames. Further exploration is needed to apply our method with point-based system for data collection.}
% \rev{}{On the other hand, since the material of the deformable surface exhibits hysteresis,} the positions of markers are captured in a quasi-static manner. As such, we \rev{always}{have to} wait \rev{}{for} 3 seconds after applying the actuation to make the system stable and then capture frames of markers. \rev{}{This represents a limitation of the proposed method when applied to robotic systems that require high dynamic performance. One possible solution is incorporating other techniques that can handle sequential data inputs in the learning pipeline (e.g.,~\cite{Thuruthel2017DynamicsLearning}).}

% \subsubsection{\rev{}{Design of deformable mannequin}}
% The design of the proposed deformable surface can be further enhanced. \rev{}{This includes optimizing the shape and location of pneumatic-driven chambers, as well as the geometry of the rigid core.} In our current design, we employed a neural distance field based method~\cite{DeepSDF2019} to determine a volumetric region that is commonly `inside' the body shapes of all individuals. \rev{}{We have not considered the poses of individuals when determining the shape of the core. We plan to address this limitation in our future work.}


%\TianModify{}{The deformable mannequin, as detailed in Sec.\ref{secSoftMannequin}, combined with the proposed sim-to-real learning method, enables precise shape control of free-form surfaces, allowing it to serve as a reusable 3D mold for sustainable garment fabrication.}
%
%\TianModify{}{Pproof-of-concept experiments were conducted to verify the feasibility of this approach in collaboration with the Dutch startup NEFFA~\cite{morby2016}. As illustrated in Fig.\ref{fig:GarmentFabrication}(a), the soft robotic mannequin is deformed to the calculated shape, after which a biodegradable material is applied to the surface. This material begins with the introduction of water, sugars, and minerals into a bioreactor along with tiny particles of mycelium. Over a period of 3 to 7 days, depending on the size of the bioreactor, the mycelium grows. Once harvested, additional ingredients and pigments are added to produce the final material.}
%
%\TianModify{}{During the fabrication process, as shown in Fig.\ref{fig:GarmentFabrication}(b), a thermal camera monitors the procedure until the temperature stabilizes across the whole surface (Fig.\ref{fig:GarmentFabrication}(c)), indicating that the mycelium layer has fully formed. The garment is then cut along the designated curve and carefully taken off, as illustrated in Fig.\ref{fig:GarmentFabrication}(d). The completed waistcoat is subsequently ready for wear, as displayed in Fig.\ref{fig:GarmentFabrication}(e). Notably, the soft robotic mannequin’s surface remains clean throughout, ensuring it is reusable for future applications.}
%
%\TianModify{}{In summary, this novel approach facilitates on-demand, true-fit garment production by adapting to individual 3D shapes and applying biodegradable materials to its surface. It also addresses waste associated with traditional garment sizing systems, which oversimplifies complex body geometries into single representative values~\cite{ellenmacarthur2017new, GuardianMeaninglessSizing}.}

%%%After discussion, this discussion should be discard
% \subsubsection{Applicability to analytical models}
% \TianModify{}{In this paper, the proposed sim-to-real method is adaptable to various numerical simulations. Consequently, extending our method to accommodate analytical models presents an interesting potential direction. In summary, our method can incorporate analytical models, provided these models offer parameterization along their deformed bodies, as our approach begins in the robot's parametric domain. For robots with only parameterization along the body (e.g., piecewise constant curvature (PCC) model \cite{webster2010design}), additional parametric dimensions can be introduced in the circular direction, transforming the parametric domain into higher DoFs, which would help address the issue. At the same time, these extra DoFs would be concatenated after the control points as conditional code for the input of $\mathcal{N}_{rbf}$ as shown in Fig.\ref{fig:comparisonSim2RealPipelines}(b). As such, the learned $\mathcal{N}_{rbf}$ can output different function variables with the same simulation shapes. This modification can transfer the points along the body, which are with the same 3D locations but different circular parameters, to different $\mathbf{p}^*$ after space warping. }


%\subsubsection{Limitation}
%\TianModify{}{Although the proposed sim-to-real network accurately models the free-form surface deformations compared to different simulation methods, some limitations remain. One main limitation is the effectiveness of our method highly relies on the quality of the training data which can cover the majority of the deformation pattern. While our sim-to-real method is capable of utilizing small and incomplete datasets to bridge the reality gap, its ability to accurately capture deformation patterns diminishes when a significant portion of the data is missing. In such cases, the extensive extrapolation required reduces the network's reliability and performance. Additionally, training our sim-to-real network demands highly accurate data due to the complex geometries it needs to learn, especially given the use of a small dataset for training. Another limitation is our method struggles to learn the surface shapes with sharp features, which comes from the fact that RBFs are inherently smooth and continuous, making them better suited for modeling smooth deformation instead of sharp edges and corners. To this end, the architecture of our sim-to-real pipeline can be modified based on the idea of binary space partitioning (BSP) Network \cite{chen2020bsp} in the future to tackle this challenge.}


==> tex/secSim2RealLearning.tex <==
\section{Learning for Sim-to-Real Transfer}\label{secSim2Real}
This section introduces our function based sim-to-real learning for shape prediction. Given a set of points $\{ \mathbf{p} \in \mathbb{R}^3 \}$on the free-form surface of a simulated model $\mathcal{S}$, we propose a method to learn a network $\mathcal{N}_{s2r}$ that can predict a deformation function mapping these points onto a corrected model $\mathcal{S}^*$ (i.e., the corrected shape that has eliminated the sim-to-real gap). The shape difference between $\mathcal{S}^*$ and the physical shape $\mathcal{S}^p$ should be minimized by the sim-to-real transfer. $\mathcal{N}_{s2r}$ is expected to be a general network\footnote{\JENew{Different networks still need be trained for different soft robotic setups.}} that can adaptively handle different simulated shapes as input.

\subsection{RBF-based Spatial Warping}\label{subsecRBFSpaceWarping}
Considering the gap between the simulated shape $\mathcal{S}$ and the physical shape $\mathcal{S}^p$, we propose to model it as a continuous spatial warping by the \textit{radial basis functions} (RBF) as follows. 
\begin{equation}\label{eqRBFSpaceWarping}
 \mathbf{p}^* = \bm{\Phi}(\mathbf{p}) = \bm{\alpha}_0 + A \mathbf{p} + \sum_{i=1}^N \bm{\beta}_i e^{-c\| \mathbf{p} - \mathbf{q}_i \|^2} 
\end{equation}
with $N$ being the number of kernels employed for the space warping and $A = [\bm{\alpha}_1, \bm{\alpha}_2, \bm{\alpha}_3]$. The centers of Gaussian kernels, $\{ \mathbf{q}_i \}$, are sparsely selected to cover the entire surface of a simulated model. The value of coefficient $c$ controlling the width of the Gaussian kernel is chosen as $3.0 \times 10^{-5}$ by experiments. We remark that $\bm{\gamma} = [\bm{\alpha}_0, \bm{\alpha}_1, ...  \bm{\beta}_i]$ are variables of function space, which can be determined by solving a linear system \cite{Charlie2007RBFVolPara}. \JENew{The kernel centers $\{ \mathbf{q}_i\}$ are selected on the simulated models according to the location of \textit{real} markers (when using a motion capture system) or \textit{virtual} markers (while employing a 3D scanner)}, where the free-form surface of a simulated model has been parameterized into $u,v$-domain and represented by a B-spline surface\JENew{~(details given in Sec.~\ref{subsecBSplineBasedRep})}. The same marker on different simulated models will have the same $(u, v)$ parameters. \JENew{Additionally, the compatibility conditions are incorporated to provide better shape control in the function space, ensuring a smooth sim-to-real mapping (see Sec.~\ref{subsecCompatibilityLoss} for details).}
% \begin{equation}\label{eqCompatibilityCondition}
% \sum_{i=1}^N \bm{\beta}_{i} 
% =\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{x}
% =\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{y}
% =\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{z}
% = \mathbf{0}
% \end{equation}

\begin{figure}[t] 
\centering
\includegraphics[width=1.0\linewidth]{fig/figSpaceWraping.jpg}\\
\vspace{-2pt}
\caption{ 
The space warping $\mathbf{\Phi}(\cdot)$ is built on the \textit{radial basis functions} (RBF) with kernel centers located on the free-form surface of a simulated model. Different warping functions are needed for different simulated shapes. 
%\Tian{font changed}
}\label{fig:spaceWarpingBackup}
\end{figure}

%\charlie{Baseline: learning for markers predictions (with figure illustration added)}
With a determined warping function $\bm{\Phi}(\mathbf{p})$, we are able to map any point $\mathbf{p} \in \mathcal{S}$ to its corresponding point $\mathbf{p}^* \in \mathcal{S}^*$ as demonstrated in Fig.\ref{fig:spaceWarping}. However, different warping functions need to be employed for different simulated shapes. A straightforward solution is to train a network $\mathcal{N}_{mk}$ to predict the positions of physical markers using the set of simulated marker positions as $\{ \mathbf{q}^* \}=\mathcal{N}_{mk}(\{ \mathbf{q} \})$. After that, the predicted positions of the physical markers and the positions of the virtual markers can be used to determine the value of $\bm{\gamma}$ and therefore also the warping function. However, there are two major problems with this straightforward sim-to-real strategy:
\begin{itemize}
\item This is not an end-to-end approach as it needs to solve a linear equation system when establishing a warping function for each simulated shape;

\item Training the marker prediction network $\mathcal{N}_{mk}$ needs sets of fully captured markers, which can be challenging on largely deformed models as discussed above.
\end{itemize}
A function space learning-based method is introduced below to solve these issues. 
%\JENew{Specifically, a network $\mathcal{N}_{rbf}$ is introduced to predict the value of the function variable $\bm{\gamma}$ according to the simulated shape $\mathcal{S}$.}
All frames of motion capture data -- even those in the presence of missing markers -- can be employed for training. \JENew{Similarly, dense point clouds with missing regions can also be employed as input for sim-to-real learning.} 


\subsection{Compact Representation by B-Spline Surface}\label{subsecBSplineBasedRepBackup}
Using all sample points on the surface of $\mathcal{S}$ may introduce redundant information and therefore require a complex network for prediction. \JENew{To overcome this problem, we first convert the freeform surface $\mathcal{S}$ of a soft deformable robot into a B-spline surface representation through 1) the parametrization taken at its rest shape (see Fig.\ref{fig:BSplineFitting}(a-c) for an example) and 2) the surface fitting conducted at every deformed shapes to determine control points of B-spline surface (denoted by $\mathcal{S}^c$ and see Fig.\ref{fig:BSplineFitting}(d)). The control points and B-Spline surfaces for three different soft robots are given in Fig.\ref{fig:BSplineFitting}(e).} 
We then employ the control points of B-spline surface $\mathcal{S}^c$ as the shape descriptor of $\mathcal{S}$, with which any point in the parametric domain with the parameter $(u_p,v_p)$ can be mapped to a point $\mathbf{p} \in \mathbb{R}^3$ as $\mathbf{p}=\mathbf{B}(u_p,v_p,\mathcal{S}^c)$. This function $\mathbf{B}(\cdot)$ is named as the B-spline based shape decoder in our computational pipeline (illustrated as the green block in Fig.\ref{fig:comparisonSim2RealPipelines}). 


%In this work, we apply B-spline surface representation as a compact shape descriptor for each free-form surface $\mathcal{S}$ generated by simulation. Specifically, the triangular mesh of $\mathcal{S}$ can be approximated by a B-spline surface, with its control points $\mathcal{S}^c$ determined through parameterization and fitting steps (see Fig. \ref{fig:BSplineFitting} for an illustration). 
The dimension of $\mathcal{S}^c$ using B-spline representation is much lower than mesh representation. For example, we use $30 \times 30$ control points for a mannequin robot as shown in Fig.\ref{fig:BSplineFitting}(d). %Note that the parameterization is consistent among all models as they are generated by numerical simulation using the mesh representation with the same set of vertices and elements -- only the positions of vertices are changed.
\JENew{Note that, since the surfaces obtained via simulation retain an unchanged mesh topology -- preserving correspondence -- the B-spline surface fitting computation is based on the parameterization determined by the rest shape of $\mathcal{S}$.}
\begin{figure}
\centering
%\captionsetup{skip=5pt}  % Set the desired skip value
\includegraphics[width=1.0\linewidth]{fig/figParaFitting.jpg}
\caption{\JENew{The steps for generating the parameterization of a free-form surface are (a) cutting, (b) tracing the boundary, (c) flattening \cite{floater2003mean} and (d) fitting with the resultant control points. The B-Spline surfaces and control points of four different soft robots tested in this paper are given in (e).}
\Tian{Update this figure to add compression robot}
}\label{fig:BSplineFittingBackup}
\end{figure}


\begin{figure}
\centering
% \includegraphics[width=1.0\linewidth]{fig/figSpaceWraping.jpg}\\
\includegraphics[width=1.0\linewidth]{fig/figSim2Real-Pipelines.jpg}\\
\vspace{-5pt}
\caption{\JENew{With the help of B-Spline based compact representation of freeform surfaces, we propose a function-prediction based pipeline that can resiliently conduct the sim-to-real learning even when the input is in the presence of missing markers. The sim-to-real network $\mathcal{N}_{s2r}$ is formed by the components enclosed in the dash lines.}
\TianModify{}{Furthermore, to generalize our approach to point clouds or scans—where correspondences are unknown and regions may be missing—we introduce a differentiable registration module. This module jointly learns both the correspondences and the underlying function space, aided by a confidence network and multiple loss terms.}
\Tian{This figure and the section III might need re-arrangement}
}\label{fig:comparisonSim2RealPipelinesBackup}
\end{figure}


\subsection{NN-based Deformation Function Learning}\label{subsecNNBasedDefField}
%Only learning to predict the positions of markers does not provide good shape control in the regions between markers, which relies on dense and complete sets of captured markers as input to train $\mathcal{N}_{mk}$. In contrast, we propose a pipeline based on function prediction that is end-to-end after training. Moreover, 

Our function-prediction based sim-to-real pipeline is formed by three building blocks: 1) the network $\mathcal{N}_{rbf}$, 2) the B-spline based shape decoder and 3) the RBF-based space warping (i.e., Eq.(\ref{eqRBFSpaceWarping})). The diagram has been shown in Fig.\ref{fig:comparisonSim2RealPipelines}. When actuating the deformable robot into different shapes $\{ \mathcal{S}_j \}$ by $\{ \mathbf{a}_j \}$, the function-prediction network $\mathcal{N}_{rbf}$ can be trained by the positions of all captured markers $\mathbf{q}_{i,j}$ together with their corresponding parameters $(u_i,v_i)$ and the control points $\mathcal{S}^c_j$. Here $\mathbf{q}_{i,j}$ denotes the position of the $i$-th marker captured on the $j$-th frame. The loss function for learning $\mathcal{N}_{rbf}(\cdot)$ is defined as 
\begin{equation}\label{eqS2RLoss}
\mathcal{L}_{s2r} = \sum_j \sum_i \| \bm{\Phi}_j(\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)) - \mathbf{q}_{i,j} \|^2
\end{equation}
with the function variable $\bm{\gamma}$ of $\bm{\Phi}_j$ predicted by the network as $\bm{\gamma}=\mathcal{N}_{rbf}(\mathcal{S}^c_j)$ and the kernel centers of $\bm{\Phi}_j$ given as $\{ \mathbf{B}(u_i,v_i,\mathcal{S}^c_j) \}$. 
\JENew{This formulation does not require every markers -- no matter using motion capture system or 3D scanner -- to be captured, which therefore supports resilient sim-to-real learning.}
%Only captured markers are included to evaluate the loss $\mathcal{L}_{s2r}$ defined in Eq.(\ref{eqS2RLoss}). This pipeline supports resilient sim-to-real learning that can use all frames of captured data by motion camera. 

Given a well trained network $\mathcal{N}_{rbf}(\cdot)$, the sim-to-real transfer can be evaluated by the pipeline of Fig.\ref{fig:comparisonSim2RealPipelines} in the inference phase as a network $\mathcal{N}_{s2r}(\cdot)$ that gives
\begin{equation} \label{eqSim2RealPrediction}
\mathbf{p}^*=\mathcal{N}_{s2r}(\mathbf{B}(u_p,v_p,\mathcal{S}^c(\mathbf{a})),\mathcal{S}^c(\mathbf{a}),\{ \mathbf{B}(u_q,v_q,\mathcal{S}^c(\mathbf{a})\}).
\end{equation}
$(u_p,v_p)$ denotes a point sampled in the parametric domain of the free-form surface.  $\{\mathbf{B}(u_q,v_q,\mathcal{S}^c(\mathbf{a})\}$ denotes the set of marker points, which are defined by their parameters $(u_q,v_q)$ and work as kernel centers for the RBF-based warping function. 
All operators in this sim-to-real pipeline is differentiable w.r.t. the actuation parameter $\mathbf{a}$. \JENew{Detail analysis can be found in Appendix \ref{AppendixDifferentiation}}. In Sec.\ref{secNNShapeCtrl}, we will present the detail of NN-based forward kinematics and the IK computing for shape control, which is based on minimizing the distance between $\mathbf{p}^*$ and its closest point on the target shape $\mathcal{S}^t$.


\subsection{Compatibility Regularization}\label{subsecCompatibilityLoss}
\JENew{
The NN-based computation pipeline, using the $\mathcal{L}_{s2r}$ loss defined above, can effectively learn the RBF-based warping function space even when markers are missing in some deformed shapes used as training samples. However, when a significant reality gap exists -- such as in cases requiring substantial deformation -- the learned high-dimensional function space may not yield a smooth shape under deformation as illustrated in Fig.\ref{fig:comptaibleLossIllustration}(a-c). Similar issues were noted in earlier RBF-based deformation research~\cite{Charlie2007RBFVolPara,turk2002modelling}. To improve shape control on deformed 3D models, the following compatibility conditions were imposed.
\begin{align}
\label{eqCompatibilityCondition}\sum_{i=1}^N \bm{\beta}_{i} 
=\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{x}
&=\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{y}
=\sum_{i=1}^N \bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{z}
= \mathbf{0}
\end{align}
}

\begin{figure}
\centering
% \includegraphics[width=1.0\linewidth]{fig/figSpaceWraping.jpg}\\
\vspace{-5pt}
\includegraphics[width=0.97\linewidth]{fig/figCompatibleLoss.jpg}
\vspace{-10pt}
\caption{
\JENew{When there is a large gap between (a) real and (b) simulated shapes, the function space-based sim-to-real learning may generate RBF warping results in a weird shape as shown in (c). This problem can be effectively solved by introducing the compatibility loss as a regularization term during training -- see (d) for the result of sim-to-real correction. The color map illustrates the distribution of geometric errors.}%\Tian{figure font changed.}
}\label{fig:comptaibleLossIllustration}
\end{figure}


\JENew{To impose similar constraint on the deformation function predicted by the network $\mathcal{N}_{rbf}$, we formulate the compatibility conditions in Eq.\eqref{eqCompatibilityCondition} as a loss function to be included during learning:}

\vspace{-10pt}
\JENew{
\begin{align}\label{eqCompatibilityLoss}
    \mathcal{L}_{c} &=  
    \|\sum_{i=1}^N \bm{\beta}_{i}\|^{2} + \|\sum_{i=1}^N\bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{x}\|^{2} + \|\sum_{i=1}^N\bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{y}\|^{2} \nonumber
\\ &+ \|\sum_{i=1}^N\bm{\beta}_{i} \left(\mathbf{q}_{i}\right)_{z}\|^{2}.
\end{align}}

\JENew{This loss serves as a regularization term to effectively penalize any nonzero combinations of function space variables. The total loss of sim-to-real training is then defined as
\begin{equation}
    L = L_{s2r} + w_c L{c}
\end{equation}
with the weight $w_c=1.5e-4$ being chosen by experiments. As a consequence, the learned function space forms a smooth and consistent subspace even under large deformations, facilitating well-controlled shapes in sim-to-real transfer (see Fig.\ref{fig:comptaibleLossIllustration}(d) for an example). Significant discrepancies between simulated and physical results are commonly seen with large inflation deformations in soft robots. By incorporating the compatibility loss, the learned mapping enhances generalization and provides more reliable performance. 
}
%\charlie{Edited (28/10)}


==> tex/secSim2RealwithDenseInput.tex <==
\section{Sim-to-Real by Point Clouds}\label{secSim2RealwithDenseInput}
\Tian{Need discussion about the way we rephrase this section}
\JENew{
The function-based sim-to-real learning method introduced above needs the corresponding positions $\mathbf{q}_{i,j}$ of every markers (denoted by $\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)$) for the $i$-th marker on the $j$-th deformed shape in Eq.\eqref{eqS2RLoss} defined on the simulated robot, though it can tolerate some missing markers in each frame. Unlike using the motion capture system where the positions and orders of markers are predefined so that the correspondences are unchanged during data acquisition for sim-to-real training, point clouds obtained from 3D scanners do not provide such correspondences. This section presents a method to obtain `virtual' markers on the simulated models and then seeks the help of rigid and non-rigid registration to rebuild correspondences for the `virtual' markers.  
}
%$\mathbf{q}_{i,j}$ denotes the position of the $i$-th marker captured on the $j$-th frame.

\subsection{Virtual Markers} 
\JENew{
All deformed shapes of a soft robot are represented by a B-Spline surface in our approach. Therefore, we are able to generate nearly uniform samples in the parametric domain of the B-Spline surface $u,v \in [0,1] \times [0,1]$ to work as `virtual' markers -- see Fig.\ref{fig:DenseInputPreprocessing} for an illustration. The corresponding positions $\mathbf{q}_{i,j}$ of a marker $\mathbf{p}_{i,j}=\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)$ on the $j$-th deformed shape will be determined via the registration process introduced below. Here $\mathcal{S}^c_j$ denotes the control points of the B-Spline surface that approximates the $j$-th deformed shape obtained from simulation.
}

%\TianModify{}{After registration described in Sec.\ref{subSecRegistration}, the relationship between the scan model and the simulation model is established. To generate sim-real pairs with proper density, we resample \cite{DownSamplingPyTorch3D} the initial point cloud of the scan model in $(u, v)$ domain with specific voxel size as shown in Fig.\ref{fig:DenseInputPreprocessing}(e). Corresponding points on the simulation model are then computed using a B-Spline representation with the same $(u_p, v_p)$ values: $\mathbf{p}=\mathbf{B}(u_p,v_p,\mathcal{S}^c)$ and the points are visualized in Fig.\ref{fig:DenseInputPreprocessing}(f). The resulting dataset of Sim-Real pairs is grouped and prepared for training, as described in Sec. \ref{secSim2Real}.} 

\begin{figure}[t] 
\centering

\includegraphics[width=1.0\linewidth]{fig/figDenseInputPreprocessing.jpg}\\
\vspace{-0pt}
\caption{
\JENew{Virtual markers are generated in the $u,v$-domain of the B-spline surface and mapped onto the 3D simulated shape (a). Given the raw scans as 3D point clouds for different frames of deformed shapes -- displayed in different colors in (b), the rigid registration is conducted by the static regions (displayed in gray) to align the coordinate systems of different frames -- see the result given in (c). With the help of non-rigid registration by deforming the scanned model onto the simulated shape (d-e), we are able to determine the positions of virtual markers on the point cloud of a scanned model (f).}\Tian{Describe two types of registration: baseline and our method}
}\label{fig:DenseInputPreprocessing}
\end{figure}

\subsection{Registration for Correspondence Retrieval}\label{subSecRegistration}
\JENew{Both rigid and non-rigid registrations are conducted on the 3D scanned point clouds. The purpose is to find the position $\mathbf{q}_{i,j} \in \mathcal{P}_j$ of every `virtual' marker $\mathbf{p}_{i,j}=\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)$ with $\mathcal{P}_j$ being the point cloud of the $j$-the frame -- i.e., determining the correspondence of $\mathbf{p}_{i,j}$ on the scanned model.} 

\subsubsection{Rigid registration for coordinate system alignment}
\JENew{
To align all frames to a common coordinate system, rigid registration is used to compute a global transformation $(\mathbf{R}_j, \mathbf{t}_j)$ between the initial frame and every rest frame $\mathcal{P}_j$. This is realized by applying the \textit{Iterative Closest Point} (ICP) algorithm \cite{ICP1992} on the static parts of scans -- as the gray regions shown in Fig.\ref{fig:DenseInputPreprocessing}(b-c). Following the strategy employed in \cite{kwok2014volumetric}, the closest points that are failed in the inverse closest check are excluded from the ICP-based registration so that enhances the stability of rigid registration. 
}

\subsubsection{Non-rigid registration for correspondence}
\JENew{
After rigid registration, for each pair of simulated and scanned models as shown in Fig.\ref{fig:DenseInputPreprocessing}(c), the correspondence between them are still unknown considering the significant difference in shape. To find the corresponding point 
$\mathbf{q}_{i,j} \in \mathcal{P}_j$ of every `virtual' marker $\mathbf{p}_{i,j}=\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)$, we conduct a step of non-rigid registration \cite{yao2020quasi} to deform $\mathcal{P}_j$ onto the simulated shape by computing an affine transformation field where each point in $\mathcal{P}_j$ is assigned with a unique affine transformation matrix. Distance and normal compatibility criteria (using the distance threshold as 0.05m and the normal variation threshold as $60^\circ$) are employed to improve the accuracy of non-rigid registration. After taking this non-rigid registration step, the scanned point cloud $\mathcal{P}_j$ is deformed into a point cloud $\mathcal{P}^*_j$ well-aligned with the simulated model as shown in Fig.\ref{fig:DenseInputPreprocessing}(e). For a virtual marker $\mathbf{p}_{i,j}=\mathbf{B}(u_i,v_i,\mathcal{S}^c_j)$, we can found its closets point $\mathbf{q}^*_c=\arg \min_{\mathbf{q}^* \in \mathcal{P}^*_j} \| \mathbf{q}^* - \mathbf{p}_{i,j}\|$. Therefore, the position of $\mathbf{q}^*_c$ before non-rigid registration gives the location $\mathbf{q}_{i,j}$ of the marker on $\mathcal{P}_j$. The correspondences can then be retrieved. Note that, when the distance between $\mathbf{q}^*_c$ and $\mathbf{p}_{i,j}$ is too big -- i.e., 2mm is employed as a threshold in our implementation, the marker $\mathbf{p}_{i,j}$ is considered as `missed' on $\mathcal{P}_j$. 
}

